Imbalance Trouble: Revisiting Neural-Collapse Geometry

Neural Collapse refers to the remarkable structural properties characterizing the geometry of class embeddings and classifier weights, found by deep nets when trained beyond zero training error. However, this characterization only holds for balanced data. Here we thus ask whether it can be made invariant to class imbalances. Towards this end, we adopt the unconstrained-features model (UFM), a recent theoretical model for studying neural collapse, and introduce Simplex-Encoded-Labels Interpolation (SELI) as an invariant characterization of the neural collapse phenomenon. Specifically, we prove for the UFM with cross-entropy loss and vanishing regularization that, irrespective of class imbalances, the embeddings and classifiers always interpolate a simplex-encoded label matrix and that their individual geometries are determined by the SVD factors of this same label matrix. We then present extensive experiments on synthetic and real datasets that confirm convergence to the SELI geometry. However, we caution that convergence worsens with increasing imbalances. We theoretically support this finding by showing that unlike the balanced case, when minorities are present, ridge-regularization plays a critical role in tweaking the geometry. This defines new questions and motivates further investigations into the impact of class imbalances on the rates at which first-order methods converge to their asymptotically preferred solutions.

==> sections/Misc.tex <==
\subsection{Weaker notion of margin-maximization}
The following lemma is along the lines of \cite[Thm.~5.2]{vardi2021margin}. The proof is similar to \cite[Thm.~5.2]{vardi2021margin} and uses the convergence result of \cite{ji2021unconstrained}. 
\begin{lemma}
Assume there exists $t_0$ such that $\Lc(\W^{t_0},\Hb^{t_0})<1$, where $(\W^{t_0},\Hb^{t_0})$ are iterates of gradient flow (GF) on the CE loss \eqref{eq:CE}. Then, the GF converges in direction to a KKT point $(\hat\W,\hat\Hb)$ of \eqref{eq:svm_original}, such that 
\begin{align}
\hat\Hb&=\arg\min_{\Hb} ~\frac{1}{2}\|\Hb\|^2\qquad\text{sub. to}\quad (\hat\w_{y_i}-\hat\w_{c})^T\h_i \geq 1 \label{eq:H_opt}
\\
\hat\W&=\arg\min_{\W} ~\frac{1}{2}\|\W\|^2\qquad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T\hat\h_i \geq 1 \label{eq:W_opt}
\end{align}
\end{lemma}

Note that both programs above are convex and Slater's conditions are satisfied. Thus, KKT conditions are necessary and sufficient for optimality in both problems. 

From the KKT conditions of \eqref{eq:H_opt}, we know (see Equation \eqref{eq:hi_KKT}) that for all $i\in[n]$, there exist $\lab_c\in\R^{k-1}, c\in[k]$ such that
\begin{align}\label{eq:hi_KKT_2}
&\hat\h_i = \hat\A_{-{y_i}}^T\lab_{y_i} 
\end{align}
and $\lab_c, c\in[k]$ are such that
\begin{align}\label{eq:hat_la}
\lab_{c}\geq \zeros,  \qquad \hat\A_{-c}\hat\A_{-c}^T\lab_c\geq \ones, \qquad \lab_{c}^T(\ones-\hat\A_{-c}\hat\A_{-c}^T\lab_c)=0
\end{align}
where $\hat\A_{c}=\ones\hat\w_c-\hat\W_{-c}^T$.

Next, we look at problem \eqref{eq:W_opt}. By the same argument as in Lemma \ref{lem:centering}, it must be that $\sum_{c\in[k]}\hat\w_c=\zeros$. Hence, Equation \eqref{eq:hat_la} holds for $\hat\A_{c}=-(\Id+\ones\ones^T)\hat\W_{-c}^T$. Also, the KKT conditions for problem \eqref{eq:W_opt} give
\begin{align}
\w_c - \sum_{i:y_i=c}\sum_{c'\neq c}\mu_{i,c'}\hat\h_i +  (K-1) \sum_{i:y_i\neq c}\mu_{i,c}\hat\h_i = 0,
\end{align}
for dual variables $\mu_{i,c}, i\in[n], c\in[k], c\neq y_i$ such that
\begin{align}
\mu_{i,c} \geq 0,\quad \mu_{i,c}\left(1 - \right)
\end{align}


==> sections/analysis.tex <==
\section{Analysis}

\begin{lemma}\label{lem:centering}
 Any global minimizer $(\hat\W,\hat\Hb)$ of \eqref{eq:svm_original} is such that $\sum_{c\in[k]}\hat\w_c=\zeros$.
\end{lemma}

\begin{proof}
For the sake of contradiction assume that $\bar\w:=\frac{1}{k}\sum_{c\in[k]}\hat\w_c\neq \zeros$, that is $\|\bar\w\|_2>0$. Consider the pair $({\Vb},\hat\Hb)$ where the columns of $\Vb$ are defined each such that $\vb_c=\hat\w_c-\bar\w$. Clearly, the new pair is feasible, since $(\hat\W,\hat\Hb)$ is feasible. But, 
$$
\sum_{c\in[k]}\|\vb_c\|^2 = \sum_{c\in[k]}\|\w_c\|^2 + k\|\bar\w\|^2 - \inp{\bar\w}{\sum_{c\in[k]}\w_c} =  \sum_{c\in[k]}\|\w_c\|^2 - k\|\bar\w\|^2 <\sum_{c\in[k]}\|\w_c\|^2,
$$
which contradicts optimality of $(\hat\W,\hat\Hb)$. Hence, it must be that $\bar\w=\zeros$.
\end{proof}


Consider first the minimization over $\Hb$ for any fixed $\W$:
\begin{align}
\Hb(\W):=\arg\min_{\Hb}~\frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
\end{align}
Note that this optimization is separable over the rows of $\Hb$ and each row of $\Hb(\W)$ is found by minimizing the following:
\begin{align}\label{eq:hi_sep}
\min_{\h}~\frac{1}{2}\|\h_i\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1\quad\forall c\neq y_i
\end{align}
The above optimization is strongly convex. Slater's conditions hold, thus KKT conditions are necessary and sufficient. Therefore the solution $\hat\h_i:=\h_i(\W)$ of the problem  above is unique and satisfies:
\begin{align}\label{eq:hi_KKT}
\hat\h_i = \A_{-{y_i}}^T\lab_i , \qquad \lab_i\geq \zeros,  \qquad \A_{y_i}\hat\h_i\geq \ones, \qquad \lab_i^T(\ones-\A_{-{y_i}}\hat\h_i)=0
\end{align}
for some optimal dual variable $\lab_i\in\R^{k-1}$. Also, from strong duality, the minimization in \eqref{eq:hi_sep} is equivalent to the following maximization
\begin{align}
\max_{\lab} ~-\frac{1}{2}\|\A_{y_i}^T\lab\|^2+\lab^T\ones \quad\quad\text{sub. to}\quad \lab \geq 0.
\end{align}

\begin{remark}
Note that {if $\A_{y_i}\A_{y_i}^T$ is invertible and $\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\geq \zeros$,} then the primal dual pair:
\begin{align}
 \hat\h_i=\A_{y_i}^T\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones\qquad{\text{and}}\qquad\lab_i=\left(\A_{y_i}\A_{y_i}^T\right)^{-1}\ones
\end{align}
 satisfies the KKT and is thus optimal. However, this might not be true for the optimal $\W$. Thus, we consider below the general case.
 \end{remark}
 
 In general, \eqref{eq:svm_original} reduces to the following min-max optimization
 \begin{align}\label{eq:cvx_onlyW}
\min_{\substack{\W\\
\A_{y_i}=\ones\w_{y_i}^T-\W_{-y_i}^T
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\|\W\|^2 -\frac{1}{2}\sum_{i\in[n]}\|\A_{y_i}^T\lab_i\|^2 + \sum_{i\in[n]}\lab_i^T\ones.
\end{align}
From Lemma \ref{lem:centering}, the optimization above does not change when we impose the additional constraint $\sum_c\w_c=\zeros$. Using this, note that $\w_c = -\W_{-c}\ones, \forall c\in[k]$. Therefore, 
\begin{align}
\A_c = \ones\w_c^T-\W_{-c}^T = -\ones\left(\W_{-c}\ones\right)^T-\W_{-c}^T = -\left(\Id+\ones\ones^T\right)\W_{-c}^T
\end{align}
Therefore,
$$
\A_c\A_c^T = \left(\Id+\ones\ones^T\right)\W_{-c}^T\W_{-c}\left(\Id+\ones\ones^T\right).
$$
Recalling the notation of the Gram matrix $\G$ and its submatrices $\G_{-c}, c$ and recognizing that $\G_{-c}=\W_{-c}^T\W_{-c}$, we can rewrite the optimization in \eqref{eq:cvx_onlyW} as follows
 \begin{align}\label{eq:cvx_onlyG}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_i\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{i\in[n]}\lab_i^T\left(\Id+\ones\ones^T\right)\G_{-y_i}\left(\Id+\ones\ones^T\right)\lab_i + \sum_{i\in[n]}\lab_i^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W \succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \sum_{c\in[k]}\w_c=\zeros \nn
\end{align}
By symmetry, for all $i: y_i=c$ it holds that $\la_i=\la_c$. Also, note that
$$
(\W^T\W\ones = \zeros ~~\text{ OR }~~ \ones^T\W^T\W = \zeros^T) \Leftrightarrow \W\ones=\zeros.
$$
 Using these, we can further reduce the above to the following
 \begin{align}\label{eq:cvx_onlyG_c}
&\min_{\substack{\W, \G, \G_{-c}
}} ~\max_{\lab_c\geq \zeros }~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\left(\Id+\ones\ones^T\right)\G_{-c}\left(\Id+\ones\ones^T\right)\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones\\
&~~\text{sub. to}\qquad\quad \G = \W^T\W\succeq \zeros,~~ \G_{-c} = \J_c\G\J_c^T,~~ \G\ones=\zeros,~~ \ones^T\G=\zeros^T \nn
\end{align}
Finally, we can exploit the lemma below, to write the optimization only in terms of Gram matrices.
\begin{lemma}\label{lem:chol}
Consider arbitrary $\G\succeq\zeros_{k\times k}$ with $\G\ones=\zeros.$
%with $\rm{rank}(G)=r$. 
Assume $d\geq k-1$. Then, there exists $\W\in\R^{d\times k}$ such that $\G=\W^T\W$.
\end{lemma}
\begin{proof}
Recall that any positive semidefinite matrix $\G\succ\zeros_{k\times k}$ with $\rm{rank}(G)=r$ has a  Cholesky factorization $\G=\Lb\Lb^T$ with $\Lb\in\R^{k\times k}$ lower triangular with exactly $r$ positive diagonal elements and $k-r$ columns containing all zeros. Note since $\G\ones=\zeros$, $r\leq k-1$ in our case. Thus, $\Lb$ has at least one column containing all zeros. Remove that column and with some abuse of notation let $\Lb\in\R^{k\times (k-1)}$ be the remaining Cholesky factor. Then, for all $d\geq k-1$, we can choose $\W = \begin{bmatrix} \Lb^T \\ \zeros_{(d-(k-1))\times k} \end{bmatrix}$, which completes the proof.
 \end{proof}
 Indeed, using Lemma \eqref{lem:chol}, the optimziation in \eqref{eq:cvx_onlyG_c} is equivalent \footnote{Here, equivalence is in the following sense. If $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, then $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}. Also, if $\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_G}, then $\hat\W,\hat\G,\hat\G_c$ are optimal in \eqref{eq:cvx_onlyG_c}, where here $\hat\W$ is such that $\hat\W^T\hat\W=\hat\G$ and its existence is guaranteed by Lemma \ref{lem:chol}.}
  to the following:
\begin{align}\label{eq:cvx_G}
&\min_{\substack{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}
}} ~\max_{\lab_c\geq \zeros }~~F(\G,\lab_c) :=\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\widetilde\J_c\G\widetilde\J_c^T\lab_c + \sum_{c\in[k]}n_c\lab_c^T\ones,
\end{align}
where we set $\widetilde\J_c:=\left(\Id_{k-1}+\ones\ones^T\right)\J_c.$

 
 We can write the inner maximization in \eqref{eq:cvx_G} using strong duality as follows
 \begin{align}
& \min_{\mub_c\geq \zeros}\max_{\lab_c}~~\frac{1}{2}\tr(\G) -\frac{1}{2}\sum_{c\in[k]}n_c \lab_c^T\tilde\J_c\G\tilde\J_c^T\lab_c + \sum_{c\in[k]}\lab_c^T\left(n_c\ones + \mub_c\right)\\
=&\min_{\mub_c\geq \zeros}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),
 \end{align}
 where we recall that $\G_{-c}:=\J_c\G\J_c^T.$
 
 \begin{propo}\label{eq:h_opt}
 	Let $(\hat\W,\hat\Hb)$ be any global minimizer of \eqref{eq:svm_original}. Then, the Gram matrix $\hat\G:=\hat\W^T\hat\W$ is a minimizers of the following convex SDP:
 \begin{align}\label{eq:SDP}
 &\min_{\G,\G_{-c},\mub_c}~~\frac{1}{2}\tr(\G) + \frac{1}{2}\sum_{c\in[k]} \frac{1}{n_c}\left(n_c\ones + \mub_c\right)^T \left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right) 
 \\
 \nn
 &~~\text{sub. to}\quad \G\succeq \zeros_{k\times k},~~\G_{-c}=\J_c\G\J_c^T,~~\mub_c\geq\zeros_{k-1},~~\G\ones=(\ones^T\G)^T=\zeros.
 \end{align}
 Moreover, letting $\hat\mub_c, c\in[k]$ denote minimizers of the convex program above and defining $$\hat\lab_c = \frac{1}{n_c}\left(\Id - \frac{1}{k}\ones\ones^T\right) \G_{-c}^{-1} \left(\Id - \frac{1}{k}\ones\ones^T\right) \left(n_c\ones + \mub_c\right),$$
 it holds for all $i\in[n]$ that,
 $$
\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
 $$
 \end{propo}
 
 \begin{remark}
Solving \eqref{eq:SDP} in CVX gives $\hat\mub_c = 0, \forall c\in[k]$. Hence, $\lab_{c}>\zeros$, which would imply that all constraints are active. Unfortunately, we know that this is NOT true if we run GD. \red{Our conjecture (?) is that GD converges to a KKT point of \eqref{eq:SDP} that is NOT a global optimum.}
 \end{remark}
 
 \subsection{The Dual problem}

 \begin{propo}
 The dual of \eqref{eq:svm_original} is the following (convex) SDP:
 \begin{align}
& \max_{\lab_c\in\R^{k-1}, c\in[k]}~~\sum_{c\in[k]}n_c\lab_c^T\ones_{k-1}\\
& ~~~\text{sub. to}~~~~~ \lab_c \geq 0\nn\\
& \qquad\qquad\qquad \Pb_k\left(\Id_k - \sum_{c\in[k]}n_c\J_c^T\left(\Id_{k-1}+\ones\ones^T\right)\lab_c\lab_c^T\left(\Id_{k-1}+\ones\ones^T\right)\J_c\right)\Pb_k\succeq 0\nn
 \end{align}
 where we set $\Pb_k:=\Id_k-\frac{1}{k}\ones\ones.$ 
 \end{propo}

Remark: A fast way to see the above is from \eqref{eq:cvx_G}. The second constraint can be written in an SDP form using Schur complement.


\subsection{A direct tight convex relaxation}
The following program is a convex relaxation of \eqref{eq:svm_original} found by setting
\begin{align}\label{eq:X_rel}
\X_{2k \times 2k} = \begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix},
\end{align}
for $\bar\Hb_{d \times k}=[\bar\h_1, \ldots, \bar\h_k]$ the feature matrix. Here, we note in \eqref{eq:svm_original} that at the optimal $\h_i=\bar\h_{y_i}$ for all $i\in[n].$

\begin{align}\label{eq:cvx_X2}
&\min_{\X\in\R^{{2k \times 2k}}}~~\sum_{c\in[k]}\X[c,c] + \sum_{c\in[k]}n_c\X[k+c,k+c]\\
&~\text{sub.~to}~~~~\X[c,k+c]-\X[c',k+c]\geq 1,~c'\neq c, c\in[k] \\
&\qquad\qquad\quad\X\succeq 0_{2k\times 2k}
\end{align}

It is not hard to see that the relaxation is tight provided that $d\geq 2k$ \ct{(This is loose. The $\X$ matrix is not gonna be full rank at the optimal. For example, we can add without loss of generality the constraint that row-column sum of top $k\times k$ block is $0$)}. Indeed, for any $d\geq 2k$, we can decompose an optimal $\hat\X$ in factors $\hat\W$ and $\hat\Hb$ using Cholesky decomposition (see Lemma \ref{lem:chol}). It is easy to verify that these factors $\hat\W$ and $\hat\Hb$ are feasible in \eqref{eq:cvx_G}. Hence they are optimal.


 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%% December 6 -- optimize first over G, then over \la
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \subsection{Old}
%% Interestingly, the min-max problem in \eqref{eq:cvx_G} is convex-concave. {Also, it should be possible (check?) to show that the minimization can be equivalently performed in a bounded set.} Thus, by Sion's min-max theorem, we can flip the order of min-max. 
%%
%%For convenience, denote $\tilde\J_c:=\left(\Id+\ones\ones^T\right)\J_c$, $c\in[k].$ The objective can be written as 
%%$$
%%F(\G,\lab_c)= \frac{1}{2}\tr\left(\G \X \right) + \sum_{c\in[k]}n_c\lab_c^T\ones,
%%$$
%%where we defined
%%\begin{align}
%%\X := \Id - \sum_{c\in[k]} n_c \tilde\J_c^T\lab_c\lab_c^T\tilde\J_c.
%%\end{align}
%%
%%\begin{lemma}\label{lem:Gmin}
%%The following is true about the minimization over $G$:
%%\begin{align}
%%\min_{\substack{\G \succeq \zeros \\ \G\ones=\zeros,~ \ones^T\G=\zeros^T}}\tr\left({\G\X}\right)=\begin{cases}
%%0 & \Pb^\perp_k\X\Pb^\perp_k\succeq \zeros \\
%%-\infty & \text{o.w.}
%%\end{cases}
%%\end{align}
%% \end{lemma}
%% Using Lemma \ref{lem:Gmin}, \eqref{eq:cvx_G} is reduces to the following maximization
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad \sum_{c\in[k]}n_c\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)\left(\Pb^\perp_k \tilde\J_c^T\lab_c\right)^T\preceq \Pb^\perp_k
%% \end{align}
%% Using Schur-complement, we can write this as an SDP:
%% \begin{align}
%% \max_{\lab_c\geq \zeros}~ \sum_{c\in[k]}n_c\lab_c^T\ones 
%% \qquad\text{sub. to}\quad 
%% \begin{bmatrix} 
%%\Id_{k\times k}  & \sqrt{n_1}\tilde\J_1^T\lab_1 & \sqrt{n_2}\tilde\J_2^T\lab_2 & \cdots & \sqrt{n_k}\tilde\J_2^T\lab_2 \\
%% \sqrt{n_1}\lab_1^T\tilde\J_1  & 1 & 0 & \cdots & 0 \\  \sqrt{n_2}\lab_2^T\tilde\J_2  & 0 & 1 & \cdots & 0 \\  
%%\vdots & \vdots & \vdots & \cdots & \vdots \\
%%\\  \sqrt{n_k}\lab_k^T\tilde\J_1  & 0 & 0 & \cdots & 1  
%%  \end{bmatrix} \succeq \zeros_{2k \times 2k}
%% \end{align} 




%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\subsection{KKT conditions}
The Lagrangian of the convex problem of \eqref{eq:svm_original} is the following, for dual variables $\{\la_{i,c}\}, i\in[n], c\in[k], c\neq y_i$:
\begin{equation}
	\Ellc(\W, \Hb, \{\lambda_{i,c}\}) = \frac{1}{2}\sum_{c=1}^{K}\|\w_{c}\|^2+ \frac{1}{2}\sum_{i=1}^{N}\|\h_{i}\|^2 + \sum_{i\in[n]}\sum_{c'\neq y_i}\la_{i,c'}(1-\w_{y_i}^T\h_{i}+\w_{c'}^T\h_i)
\end{equation}
The KKT conditions are then as follows:
\begin{subequations}\label{eq:KKT}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}+\sum_{i:y_i\neq c}\la_{i,c}\h_i -\sum_{i:y_i=c}\Big(\sum_{c'\neq y_i} \la_{i,c'}\Big)\h_i = 0\\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{i\in[n]}\Big(\sum_{c'\neq y_i}\lambda_{i,c'}\Big)\w_{y_i}+\sum_{i\in[n]}\sum_{c'\neq y_i}\lambda_{i,c'}\w_{c'} = 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\lambda_{i,c} \geq 0\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \lambda_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}

The KKT conditions can be rewritten equivalently with respect to an augmented dual variable representation $\beta_{i,c}, i\in[n], c\in[k]$ as follows:
\begin{subequations}\label{eq:KKT_beta}
\begin{align}
	\forall c\in[k]\,&:\,\nabla_{\w_{c}}\Ellc = \w_{c}-\sum_{i\in[n]}\beta_{i,c}\h_i  = 0 \,\Leftrightarrow\,  \W_{d\times k} = \Hb_{d\times n}\Bb^T_{n\times k} \\
	\forall i\in[n]\,&:\,	\nabla_{\h_i}\Ellc = \h_{i}-\sum_{c\in[k]}\beta_{i,c}\w_c = 0\,\Leftrightarrow\,  \Hb_{d\times n} = \W_{d\times k}\Bb_{k\times n} \\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,\beta_{i,c} \leq 0 \label{eq:beta_new}
	\\
	\forall i\in[n] \,&:\,\beta_{i,y_i} = -\sum_{c\neq y_i}\beta_{i,c}\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\,	\w_{y_i}^T\h_{i}-\w_{c}^T\h_{i}\geq 1
	\\
	\forall i\in[n], c\in[k], c\neq y_i\,&:\, \beta_{i,c}(1-\w_{y_i}^T\h_{i}+\w_{c}^T\h_{i}) = 0
\end{align}
\end{subequations}
To see that these are equivalent, set for all $i\in[n]$: $\beta_{i,c}=\begin{cases} \sum_{c'\neq c}\lambda_{i,c'} & c=y_i \\ -\lambda_{i,c} & c\neq y_i\end{cases}.$ Above, we have also defined an $k\times n$ matrix $\Bb$ with entries $[\Bb]_{c,i}=\beta_{i,c}.$ From constraint \eqref{eq:beta_new} it follows that $\Bb$ has column-sum equal to zero, i.e. $\Bb^T\ones_{k}=0.$ For instance this immediately yields $\W\ones_{k}=0$ (which we proved from first principles in Lemma \ref{lem:centering}).

Also, note that the first two conditions imply
\begin{align}
\Hb^T\W = \Hb^T\Hb \Bb^T \qquad\text{and}\qquad \W^T\Hb = \W^T\W\Bb.
\end{align}
Hence,
\begin{align}
\X_{(k+n)\times (k+n)}:=\begin{bmatrix}\W^T\W & \W^T\Hb \\ \Hb^T\W & \Hb^T\Hb\end{bmatrix}=\begin{bmatrix}\W^T\W & \zeros_{k\times n} \\ \zeros_{n\times k} &\Hb^T\Hb\end{bmatrix}
\underbrace{\begin{bmatrix}\Id_{k\times k} & \Bb_{k\times n} \\ \Bb^T_{n\times k} & \Id_{n\times n}\end{bmatrix}
}_{\widetilde{\Bb}}.
\end{align}
and
\begin{align}
\tr\Big(\widetilde{\Bb}^T\X \Big) = \tr\Big(\widetilde{\Bb}\cdot {\rm{bldiag}}(\W^T\W,\Hb^T\Hb) \cdot\widetilde{\Bb}\Big)
\end{align}




%A possibly interesting observation here is the following.
%\begin{lemma} Suppose $(\W,\Hb,\Bb)$ satisfy the KKT conditions \eqref{eq:KKT_beta}. If $\Bb$ is such that $\Id_{k\times k} \succeq \Bb\Bb^T$, then the matrix $\X=\begin{bmatrix} \W^T \\ \bar{\Hb}^T \end{bmatrix} \begin{bmatrix} \W & \bar\Hb \end{bmatrix}$ is a solution to the SDP in \eqref{eq:cvx_X}.
%\end{lemma}




==> sections/appx_Additional_Details.tex <==
%\ctAT{Vala,Tina}{Here please add any more details on implementation issues that did not go in the main body. For example, we should say that we based our code on the code of \citet{NC}. Also add citation to their github or whatever. If you used a sampler for imblalance data from some other code, please make sure to also add reference to that too.} \newline

% Experimental code on deep learning models are based on the code provided by the authors of of \citet{NC} with the addition of imbalanced data samplers based on the work of \citet{ImbalanceCodeRef}.  

Our experiments on deep models build on the code provided by \cite{NC}\footnote{\url{https://colab.research.google.com/github/neuralcollapse/neuralcollapse/blob/main/neuralcollapse.ipynb}}. We train ResNet-18 \cite{he2015deep} and VGG-13 \cite{vgg} models, on three 10-class datasets, CIFAR10, MNIST and Fashion-MNIST. \red{Following \cite{NC}, we use batch normalization in place of the dropout layers in VGG-13.} For both models, we disable the biases of all the fully-connected layers, similar to the experiments on UFM. We adopt the same training strategy as \cite{NC}, namely SGD on CE loss, with momentum ($0.9$), small weight decay ($5\times10^{-4}$), and learning rate $0.1$ decayed at two stages (epochs $120$ and $240$) by a factor of 10. We train the network on a $(R,1/2)$-STEP imbalance setting. To create imbalanced data, we use the data sampler provided by \citet{TengyuMa} \footnote{\url{https://github.com/kaidic/LDAM-DRW}}. Following \cite{NC} we do not use any data augmentation. In all the experiments, we fix the first 5 classes to be majorities, and the rest as minorities. To have a fair comparison between the models with different imbalance ratios $R$, we sample the datasets to have $n=25250$ training images in all cases. While the training set is imbalanced, when measuring test performance of a trained model we do so on a balanced test set, e.g. just like \cite{byrd2019effect,TengyuMa}. We measure the metrics at certain epochs, and similar to \cite{NC}, we sample epochs more frequently at the start of the training as the network parameters change more quickly in the beginning.
%\tina{after disabling the biases in their fully-connected layers}

==> sections/appx_SELI_vs_ETF_Metrics.tex <==
Recall from Definition \ref{def:SELI} that the SELI property
%When SELI property holds, Theorem \ref{thm:SVM} demonstrates how 
%relates the structure of classifiers and embeddings (namely $\G_\W:=\W^T\W$, $\G_\Hb=\Hb^T\Hb$, and $\Z=\W^T\Hb$) to the corresponding SEL matrix. Also recall that the SELI property is in general different from the ETF property.  

\Fig~\ref{fig:intro_CIFAR}
computes the distances of $\G_\W:=\W^T\W$, $\G_\Hb=\Hb^T\Hb$, and $\Z=\W^T\Hb$ , from the SELI and ETF geometries. We do this as follows.
%, at each epoch, from the corresponding decomposition given by SVD of either $\Z_{\text{ETF}}$ and $\Z_{\text{SELI}}$. 
First, for sake of memory and computation efficiency, given the good convergence with regards to the NC property in \Fig~\ref{fig:NC}, at each epoch, we only keep track of the embedding class means $\mub_c$, to represent the embeddings geometries. Additionally, we center those class means by their (balanced) global mean, i.e. we compute for each $c\in[k]:$
$$
\overline{\mub_c} = \mub_c - \mub_G,\quad\text{with $\mub_G = \frac{1}{k} \sum_{c \in [k]} \mub_c$.}
$$
Note here that the chosen centering $\mub_G=\frac{1}{k} \sum_{i\in[n]}\frac{1}{n_{y_i}}\h_i$ is in general different (and the same only when classes are balanced) from the global centering $\h_G:=\frac{1}{n}\sum_{i\in[n]}\h_i$ used by \citet{NC}. Our choice of the former is motivated by the property of the SELI geometry in \eqref{eq:center_mu}. Specifically, this choice ensures that $\sum_{c\in[k]}\overline{\mub_c}=0$ in agreement with   \eqref{eq:center_mu}. \footnote{The discrepancy between the UFM solutions being already centered, while deep-net embeddings require centering before computation of geometric measures is a common denominator in all previous works on the UFM, e.g.  \cite{zhu2021geometric,ULPM,fang2021exploring,han2021neural,lu2020neural,mixon2020neural,graf2021dissecting,zhou2022optimization}.}
%\begin{align*} 
%	 &\mub_c \in \mathbb{R}^{d}, \; \; \mub_c = \frac{1}{n_c} \Sigma_{i} \h_{i,c},\\ 
%	&\mub_G = \frac{1}{k} \Sigma_{c \in k} \mub_c, \; \; \; \; \overline{\mub_c} = \mub_c - \mub_G.
%\end{align*} 
Therefore, in all our calculations regarding the SELI and ETF convergence of embeddings, we use the centered features $\overline{\mub_c}, c\in[k]$. Overall, at each epoch, we keep track of the following feature and weight matrices
\begin{align*} 
\W = [\w_1, \w_2, ..., \w_k] \in \mathbb{R}^{d \times k}, \qquad\text{and}\qquad\M = [\overline{\mub_1}, \overline{\mub_2}, ..., \overline{\mub_k}]\in \mathbb{R}^{d \times k},
\end{align*}
with which we compute $\G_\W=\W^T\W$, $\G_\M=\M^T\M$ and $\Z=\W^T\M.$ For each such measurement, we then compute distance to reference SELI and ETF quantities $\hat\G_\W, \hat\G_\M$ and $\hat\Z$ as described in the first paragraph in \Sec~\ref{sec:rel}.
%To evaluate the distance, we compute Frobenius norm of normalized differences of the matrices, specifically we measure the distance of $A$ and $\hat{A}$ by, \begin{align*}
%    \bigg\| \frac{A}{\|A\|_F} - \frac{\hat{A}}{\|\hat{A}\|_F} \bigg\|_F.
%\end{align*}

\Fig~\ref{fig:intro_CIFAR} shows for a wide range of imbalance ratios, that the SELI geometry  describes satisfactorily the structure learned in a deep network trained till zero training error. On the other hand, the ETF characterization fails to provide an accurate approximation; note that the approximation is particularly bad for the classifier weights (i.e. for $\G_\W$.) 





% Given the convergence of NC property (\textbf{Figure 11}), we will continue to use the embedding class means to represent the feature geometries.
% \begin{align*} 
% 	 \mub_c \in \mathbb{R}^{d}, \; \; \mub_c = \frac{1}{n_c} \Sigma_{i} \h_{i,c}
% \end{align*} 
% For our calculations, we center the class embeddings by the balanced global embeddings mean.
% \begin{align*} 
% 	\mub_G = \frac{1}{k} \Sigma_{c \in k} \mub_c, \; \; \; \; \overline{\mub_c} = \mub_c - \mub_G
% \end{align*} 
% All our calculations regarding the SELI and ETF convergence of embeddings will use the centered features. From here we will have the feature and weight metrices.
% \begin{align*} 
% \W \in \mathbb{R}^{d \times k}, \; \; \; \;  \W = [\w_1, \w_2, ..., \w_k] \\
% \M \in \mathbb{R}^{d \times k}, \; \; \; \;  \Hb = [\overline{\mub_1}, \overline{\mub_2}, ..., \overline{\mub_k}] \\
% \end{align*} 
% In order to compare the overall geometry of our results with the ETF and SELI structures, we calculate the gram matrix for both the weights and feature embeddings and plot the frobenius norms of the differences in \textbf{Figure 2}.
% \begin{align*} 
% 	\G_\W = \W^T\W, \; \; \;  \G_\M = \M^T\M
% \end{align*}
% In order to compare the logits, we calculate the $\Z$ matrix using the globally centered class feature means.
% \begin{align*} 
% 	\Z = \W^T\M
% \end{align*} 
% Finally, when we compare the SELI and ETF $\Z$, $\G_\W$ and $\G_\M$ with our experimental results, we normalize the matrices using Euclidean norm: $	 \| \frac{\G_{\W / \M}}{\|\G_{\W / \M}\|_2} - \frac{\Ghat_{\W / \M}}{\|\Ghat_{\W / \M}\|_2} \|_2$ 
% %\gk{above should be $\W^T\Hb$, right?}

==> sections/appx_cifar4.tex <==
%To aid exact visual illustration of convergence to SELI geometry, we conduct deep-net training over 4 classes of CIFAR10 dataset. 
In order to illustrate the geometry for another value of the number of classes $k$, we conduct experiments over 4 classes of the CIFAR10 dataset. We consider a $(R,\nicefrac{1}{2})$-STEP imbalanced CIFAR10 dataset with only the first 4 classes used. We fix the first 2 classes to be majorities, and the rest as minorities. Other implementation details are identical to that described in \Sec~\ref{subsec:app_implementation_details}.

\Fig~\ref{fig:appx_CIFAR4_errors} shows how the distances to SELI and ETF for the classifiers, (centered) mean-embeddings, and logits evolve during training for different values of $R$. In case of the classifiers and logits, convergence to the SELI geometry is better compared to the ETF geometry. However, we note also that the convergence is worse for the embeddings compared to classifiers and logits, which in this case has a larger distance to the SELI than the ETF. \Fig~\ref{fig:appx_CIFAR4_norm_errors} illustrates the corresponding norm ratios \nicefrac{$\|\w_\text{major}\|_2$}{$\|\w_\text{minor}\|_2$} and \nicefrac{$\|\mub_\text{major}\|_2$}{$\|\mub_\text{minor}\|_2$} averaged over all pairs of majority and minority classes. Behaving similarly to the Frobenius-norm metric of \Fig~\ref{fig:appx_CIFAR4_errors}, the norm-ratios of the classifiers converge close to that of SELI, whereas this convergence is worse for the mean-embeddings.  

%To visualize the classifiers and embedding means, we construct the normalized Gram matrices $\G_\W$ and $\G_\M$ from the network weights for each epoch. Further, we compute a representative set of vectors in ($d=3$)-dimensional space $\w_1,...,\w_4 \in \Rc^{d=3}$ and $\mu_1,...,\mu_4 \in \Rc^{d=3}$ as described in Theorem \ref{thm:SVM}, with $\R= \Id_3$. 
%For comparison, we obtain the classifiers and embeddings for the corresponding ETF geometry following the same procedure with $\R = \Id_3$. 
%Figure \ref{fig:appx_CIFAR4_geom} shows the geometries of classifiers and embeddings for $R=10$, as an example. Consistent with the error plots, the classifiers can be seen converging to SELI, while the embeddings did not converge as well as the classifiers. 



\begin{figure*}[t]
	\centering
	\hspace{-40pt} \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (-1.4,-1.4) 
			{\includegraphics[scale=0.35]{figs/cifar4_GW_error.pdf}};
			%\node at (-1.4,-0.0) [scale=0.7]{\textbf{Classifier Convergence}};
			\node at (-1.4,-3.2) [scale=0.7]{Epochs};
			\node at (-4.1,-1.4)  [scale=0.7, rotate=90]{Distance to SELI/ETF};
		\end{tikzpicture}
		\caption{Classifiers}
	\end{subfigure}\hspace{25pt}\begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.35]{figs/cifar4_GM_error.pdf}};
			%\node at (0.0,-0.0) [scale=0.7]{\textbf{Feature Convergence}};
%			\node at (0,0.2) [scale=0.9]{\textbf{CIFAR10}};
			\node at (0,-3.2) [scale=0.7]{Epochs};
			\node at (-2.7,-1.4) [scale=0.7, rotate=90]{};
		\end{tikzpicture}
	\caption{Embeddings}
	\end{subfigure}\hspace{25pt}\begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.35]{figs/cifar4_Z_error.pdf}};
			%\node at (0.0,-0.0) [scale=0.7]{\textbf{Logit Convergence}};
			\node at (0,-3.2) [scale=0.7]{Epochs};
			\node at (-2.7,-1.4) [scale=0.7, rotate=90]{};
		\end{tikzpicture}
	\caption{Logits}
	\end{subfigure}
%	\label{fig:appx_CIFAR4}
	\caption{Distances of learned classifiers, embedding means and logits from SELI/ETF in the 4-class experiments on CIFAR10 dataset. % for \textbf{\underline{STEP-Imbalanced}} CIFAR10 and MNIST data trained far beyond zero training error, for different imbalance levels $R$.
	}
	\label{fig:appx_CIFAR4_errors}
%\end{figure*}
%
%\begin{figure*}[ht]
	\centering
	\hspace{-40pt} \begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (-1.4,-1.4) 
			{\includegraphics[scale=0.35]{figs/cifar4_tau_w_error.pdf}};
			%\node at (-1.4,-0.0) [scale=0.7]{\textbf{Classifier Convergence}};
			\node at (-1.4,-3.2) [scale=0.7]{Epochs};
			\node at (-4.1,-1.4)  [scale=0.7, rotate=90]{Distance to SELI/ETF};
		\end{tikzpicture}
		\caption{\nicefrac{$\|\w_\text{major}\|_2$}{$\|\w_\text{minor}\|_2$}}
	\end{subfigure}\hspace{25pt}\begin{subfigure}{0.3\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.35]{figs/cifar4_tau_h_error.pdf}};
			%\node at (0.0,-0.0) [scale=0.7]{\textbf{Feature Convergence}};
			%			\node at (0,0.2) [scale=0.9]{\textbf{CIFAR10}};
			\node at (0,-3.2) [scale=0.7]{Epochs};
			\node at (-2.7,-1.4) [scale=0.7, rotate=90]{};
		\end{tikzpicture}
	\caption{\nicefrac{$\|\mub_\text{major}\|_2$}{$\|\mub_\text{minor}\|_2$}}
	\end{subfigure}
	%	\label{fig:appx_CIFAR4}
	\caption{Comparison of the ratio of norms of the learned classifiers, embedding means and logits to those of SELI/ETF in the 4-class experiments on the CIFAR10 dataset. % for \textbf{\underline{STEP-Imbalanced}} CIFAR10 and MNIST data trained far beyond zero training error, for different imbalance levels $R$.
	}
	\label{fig:appx_CIFAR4_norm_errors}
\end{figure*}

\begin{figure*}[ht]
	\centering
	%
	\begin{subfigure}{0.45\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) 
			{\includegraphics[scale=0.3]{figs/cifar4_W_R_10.pdf}};
			%\node at (-1.4,-0.0) [scale=0.7]{\textbf{Classifier Convergence}};
%			\node at (0,-5) [scale=0.7]{Epochs};
			\node at (-4.1,-1.4)  [scale=0.7, rotate=90]{};
		\end{tikzpicture}\caption{Classifiers}\label{fig:appx_CIFAR4_geom_W}
	\end{subfigure}
	%
	%
	\begin{subfigure}{0.45\textwidth}
		\centering
		\begin{tikzpicture}
			\node at (0,-1.4) {\includegraphics[scale=0.3]{figs/cifar4_M_R_10.pdf}};
			%\node at (0.0,-0.0) [scale=0.7]{\textbf{Logit Convergence}};
%			\node at (0,-5) [scale=0.7]{Epochs};
			\node at (-2.7,-1.4) [scale=0.7, rotate=90]{};
		\end{tikzpicture}\caption{Embeddings}\label{fig:appx_CIFAR4_geom_M}
	\end{subfigure}
	\caption{\gk{to go}Visualization of geometry of learned classifiers and embeddings in the 4-class experiment with the CIFAR10 dataset for $R=10$.}
	\label{fig:appx_CIFAR4_geom}
\end{figure*}


==> sections/convex_forms.tex <==
\subsection{Convex Equivalent form: Nuclear norm}\label{eq:svm_z_nuc}
\begin{align*}
	&\quad  \min_{\Z}~\|\Z\|_*
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\Z}~\left[\min_{\W,\Hb \ \text{s.t.} \ \W\Hb = \Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)\right]
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad \Z_{y_i,i}-\Z_{c,i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb,\Z}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1, \W\Hb = \Z\\
	& = \min_{\W,\Hb}~\frac{1}{2}\left(\|\W\|^2+\|\Hb\|^2\right)
	\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_{c})^T \h_{i} \geq 1
\end{align*}

%\subsection{Equality of margins/activeness of constraints:}
%\begin{center}
%	\begin{tabular}{||c ||c | c|| c | c ||} 
%		\hline
%		& BalERM-CE & BalSVM & ImbalERM-CE & ImbalSVM \\ [0.5ex] 
%		\hline\hline
%		$(\W,\Hb)$ & Equal & Active & Unequal & Active \\ 
%		\hline
%		$\Z$ & Equal & Active & Equal & Active \\ 
%		\hline
%		$\X$ &  &  &  &  \\ [1ex] 
%		\hline
%	\end{tabular}
%\end{center}


==> sections/deepnet.tex <==


We consider multiclass classification of images using deep networks in order to support our theoretical results of neural collapse under imbalances. We optimize the weights of the networks until beyond achieving zero training error. Details of the datasets, networks and training are as given below: \newline
\textbf{Datasets:} We consider the MNIST and CIFAR10  datasets under   $(R,\rho=\nicefrac{1}{2})$-STEP imbalance with different $R$.For both datasets a total of $n = 25250$ datapoints is sampled from the maj and min classes respectively in accordance to the $R$ value. We ensure that total number of datapoints across minority and majority examples is constant regardless of imbalance ratio, meaning $n^{R = 1} = n^{R = 5} = n^{R = 10} = n^{R = 100}$. Without loss of generality the first 5 classes are taken as majority classes. \newline
\textbf{Optimization:}
\textbf{Training:} A Resnet-32 model was used for training using cross-entropy loss and SGD for $350$ epochs. Initial learning rate is set to $0.1$ and annealed by a factor of 10 at epochs $120$ and $240$. Training weight decay was set to $5 \times 10^{-4}$. Models were trained on a single GPU with a dataloader batchsize of $128$.}


==> sections/different_hyperparams.tex <==
\new{
Thus far in our analysis of the UFM, we assumed same regularization strength $\lambda$ for the embeddings and classifiers; see Eqn. \eqref{eq:CE}. Here, we discuss a slight generalization allowing different regularizations $\lambda_W$ and $\lambda_H$ for the classifiers and embeddings, respectively. This is motivated by previous studies of the UFM in the literature, e.g. \cite{zhu2021geometric}. As we show, this modification does \emph{not} change the SELI geometry modulo a relative scaling factor between the embeddings and classifiers.

Concretely, consider the following slight generalization version of Eqn.~\eqref{eq:CE}:
\begin{align}\nn%\label{eq:CE_diff_reg}
	(\What_{(\la_W,\la_H)},\Hhat_{(\la_W,\la_H)}):=\arg\min_{\W,\Hb}~\Lc(\W^T\Hb) + \frac{\la_W}{2} \|\W\|_F^2+\frac{\la_H}{2}\|\Hb\|_F^2,
\end{align}
which can be more conveniently reparameterized as follows:
\begin{align}\nn
	(\What_{(\la_W,\la_H)},\Hhat_{(\la_W,\la_H)}):=\arg\min_{\W,\Hb}~\Lc(\W^T\Hb) + \sqrt{\la_W\la_H}\left( \frac{1}{{\beta}}\|\W\|_F^2+\beta\|\Hb\|_F^2\right),
\end{align}
where $\beta := \sqrt{\frac{\la_H}{\la_W}}$ and $\la_H,\la_W>0$. Now, consider the limit of vanishing regularization $\la_W \rightarrow 0, \la_H \rightarrow 0$, with a fixed finite and non-zero ratio $\beta^2=\la_H/\la_W$. Entirely analogous to Eqn. \eqref{eq:svm_original}, this leads to the a $\beta$-parameterized UF-SVM as follows:
\begin{align}\label{eq:svm_diff_reg}
	(\What_\beta,\Hhat_\beta)\in\arg\min_{\W,\Hb}~\frac{1}{2\beta}\|\W\|_F^2+ \frac{\beta}{2}\|\Hb\|_F^2
	\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1,~i\in[n], c\neq y_i.
\end{align}
Note that the UF-SVM we study in Eqn. \eqref{eq:svm_original} is a special case of the above for $\beta=1$. For general values of $\beta>0$, it is not hard to see that there is a one-to-one mapping of global solutions $(\What_\beta,\Hhat_\beta)$ of \eqref{eq:svm_diff_reg} to global solutions $(\What_\beta,\Hhat_\beta)$ of \eqref{eq:svm_original} as follows:
$$
(\What_\beta,\Hhat_\beta) = (\sqrt{\beta}\What,\frac{1}{\sqrt{\beta}}\Hhat_\beta).
$$
Hence, from Theorem \ref{thm:SVM}, it follows that the solutions of \eqref{eq:svm_diff_reg} satisfy for any $\beta>0$ the following:
$$
\What_\beta^T\Hhat_\beta=\Zhat,\quad \Hhat_\beta^T\Hhat_\beta = \frac{1}{\beta}\Ub\Lambdab\Ub^T,\quad \text{and}\quad
\What_\beta^T\What_\beta = \beta\Vb\Lambdab\Vb^T.
$$ 
Therefore, different regularization between embeddings and classifiers only affects the geometry of global minimizers of the corresponding UF-SVM (i.e., at vanishing regularization) up to introducing an extra scaling factor between the Gram matrices of embeddings and classifiers. Specifically, this only affects the relative scaling between the norms of embeddings and classifiers. 
}

==> sections/exp_lpm.tex <==
\subsection{Unconstrained Features Model}

==> sections/exp_neural_net.tex <==
\subsection{Neural Networks}
\subsubsection{Convergence to a mean across experiments}
\subsubsection{Non-Convergence to Gcvx when $R\neq 1$}
\subsubsection{Effect on test error}
\subsubsection{Progressive Variability collapse}


==> sections/exp_ufm.tex <==
\subsection{Unconstrained Features Model}
\textbf{Step Imbalance:}\\
For the purposes of discussion, in the experiments on the UFM model, we consider the following setting. The number of classes is even ($K=2m, m\in \Zc_+$). Without loss of generality, let the classes $\{1,2,...,\nicefrac{K}{2}\}$ be called the minority classes. For the model of step-imbalance, let each of the minority classes have $n_\text{min}$ examples. Further, the classes numbered $\{\nicefrac{K}{2}+1,\nicefrac{K}{2}+2,...,K\}$ be the minorities, with $n_\text{maj}=Rn_\text{min}$, where $R$ is called the (step-)imbalance ratio.\\
\textbf{Weight decay scheduling (WDS):}\\
\subsubsection{$\Z$ and $\G$ do not converge to SVM solution with unregularized CE}
In this experiment we perform GD with WDS on CE loss. Data has $4$ classes with step imbalance of $R=10$, and $1$ example in the minority classes. The initial weight decay is $10^{-2}$.

As seen from Figure \ref{fig:unregCE_G}, the error between the matrix $\G=\W^T\W$ given by GD on unregularized CE loss in the UFM model and the matrix $\hat{\G}=\What^T\What$, of the global SVM solution remains large with proceeding iterations. Therefore, the GD solution does not converge in the direction of the global SVM solution, in agreement with our argument in Proposition \ref{propo:negative}. Figure \ref{fig:unregCE_Z} also shows that the logit matrix does not converge in the direction of the simplex encoding matrix, that is a characteristic property of the global solution of the SVM. We see from Figures \ref{fig:unregCE_margins} that the margins of the GD solution are unequal.
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/NC6 G error_R_10_Loss_CE}
		\caption{$\|\frac{\G}{\|\G\|_F}-\frac{\G_\text{SVM}}{\|\G\text{SVM}\|_F}\|_F$}
		\label{fig:unregCE_G}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/NC7 Z error_R_10_Loss_CE}
		\caption{$\|\frac{\Z}{\|\Z\|_F}-\frac{\Zhat}{\|\Zhat\|_F}\|_F$}
		\label{fig:unregCE_Z}
	\end{subfigure}
	\caption{Plots showing non-convergence of GD on CE to the SVM solution.}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/qmin normalized margins for class0_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/qmin normalized margins for class1_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/qmin normalized margins for class2_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/qmin normalized margins for class3_R_10_Loss_CE}
		\caption{}
	\end{subfigure}
	\caption{Plots showing non-convergence of normalized margins with GD on CE to that of the SVM solution. Note that all the margins of the SVM solution are equal to $1$. However, the normalized margins of the GD solution are unequal.}
	\label{fig:unregCE_margins}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/margins for class0_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/margins for class1_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/margins for class2_R_10_Loss_CE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_CE_WDS/margins for class3_R_10_Loss_CE}
		\caption{}
	\end{subfigure}
	\caption{Plots showing absolute margins with GD on CE}
\end{figure*}

\subsubsection{$\Z$ converges to simplex but $\G$ DOES NOT converge to SVM solution with logit regularization without weight decay}
In this experiment we perform GD with 0 weight decay on logit-regularized CE loss with $\lambda_\text{LogReg} = 10^{-3}$. Data has $4$ classes with step imbalance of $R=10$, and $1$ example in the minority classes.

As seen from Figure \ref{fig:logregCE_no_wd_G}, the error between the matrix $\G=\W^T\W$ given by GD on unregularized CE loss in the UFM model and the matrix $\hat{\G}=\What^T\What$, of the global SVM solution remains large with proceeding iterations. Therefore, the GD solution does not converge in the direction of the global SVM solution. However, Figure \ref{fig:logregCE_no_wd_Z} shows that the logit matrix converges in the direction of the simplex encoding matrix. We see from Figures \ref{fig:logregCE_no_wd_margins} that the margins of the GD solution are equal.
\ct{Are these with decreasing WD? If not shall they be so, for ``fair" comparison to the experiments of Sec. F.1.3?}
 \ct{Plots like 8a,b, we don't need to show so many iterations when is obvious that convergence happens earlier. They look strange otherwise :)}

\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/NC6 G error_R_10_Loss_LogRegCE}
		\caption{$\|\frac{\G}{\|\G\|_F}-\frac{\G_\text{SVM}}{\|\G\text{SVM}\|_F}\|_F$}
		\label{fig:logregCE_no_wd_G}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/NC7 Z error_R_10_Loss_LogRegCE}
		\caption{$\|\frac{\Z}{\|\Z\|_F}-\frac{\Zhat}{\|\Zhat\|_F}\|_F$}
		\label{fig:logregCE_no_wd_Z}
	\end{subfigure}
	\caption{Plots showing convergence of GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-3}$ and no weight decay to a simplex solution but not the SVM solution.}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/qmin normalized margins for class0_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/qmin normalized margins for class1_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/qmin normalized margins for class2_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/qmin normalized margins for class3_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}
	\caption{Plots showing convergence of normalized margins with GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-3}$ and no weight decay to that of a simplex logit solution.}
	\label{fig:logregCE_no_wd_margins}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/margins for class0_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/margins for class1_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/margins for class2_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_logreg_CE_NO_WD/margins for class3_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}
	\caption{Plots showing absolute margins with GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-3}$ and 0 weight decay}
\end{figure*}


\subsubsection{$\Z$ and $\G$ converge to SVM solution with logit regularization}
In this experiment we perform GD with WDS on logit regularized CE loss. Data has $4$ classes with step imbalance of $R=10$, and $1$ example in the minority classes. The logit regularization parameter is $\lambda_\text{LogReg} = 10^{-6}$, while the initial weight decay is $10^{-2}$.
\gk{G converges to SVM when there is WDS for large logReg as well, but not when we start with 0 weight decay} \ct{Nice: Well then isn't it better to show these plots for the same value of $\lambda_\text{LogReg}$ as in Sec. F.1.2? For fair comparison?}
\gk{cosmetic changes tbd}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/NC6 G error_R_10_Loss_LogRegCE}
		\caption{$\|\frac{\G}{\|\G\|_F}-\frac{\G_\text{SVM}}{\|\G\text{SVM}\|_F}\|_F$}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/NC7 Z error_R_10_Loss_LogRegCE}
		\caption{$\|\frac{\Z}{\|\Z\|_F}-\frac{\Zhat}{\|\Zhat\|_F}\|_F$}
	\end{subfigure}
	\caption{Plots showing convergence of GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-6}$ to the SVM solution.}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/qmin normalized margins for class0_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/qmin normalized margins for class1_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
	\centering
	\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/qmin normalized margins for class2_R_10_Loss_LogRegCE}
	\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
	\centering
	\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/qmin normalized margins for class3_R_10_Loss_LogRegCE}
	\caption{}
	\end{subfigure}
		\caption{Plots showing convergence of normalized margins with GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-6}$ to that of the SVM solution.}
\end{figure*}
\begin{figure*}[h]
	\centering
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/margins for class0_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/margins for class1_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/margins for class2_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.25\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/UFM_LogRegCE_vanishing_lambda_WDS/margins for class3_R_10_Loss_LogRegCE}
		\caption{}
	\end{subfigure}
	\caption{Plots showing absolute margins with GD on logit regularized CE with $\lambda_\text{LogReg}=10^{-6}$}
\end{figure*}



==> sections/implicitBias.tex <==
%\subsection{Cross-entropy}
%
%\begin{propo}[simple modification of \cite{ji2021unconstrained}]
%Even with imbalances, minimizing CE loss \eqref{eq:CE} converges in direction to a KKT point of the following margin-maximization problem:
%\begin{align}\label{eq:svm_original_implicit_bias}
%\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
%\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1
%\end{align}
%\end{propo}
%
%\ct{@Ganesh: check and sketch proof}
%

\subsection{VS-loss}

\begin{propo}[simple modification of \cite{ji2021unconstrained}]
Consider minimizing the VS-loss  
\begin{align}\label{eq:VS}
\Lc(\W,\Hb) = \sum_{i\in[n]} \log\Big(1+\sum_{c\neq y_i}e^{-\Delta_{y_i}(\w_{y_i}-\w_c)^T\h_i}\Big).
\end{align}
Then, gradient descent iterates CE loss \eqref{eq:CE} converges in direction to 
\begin{align}\label{eq:cssvm_original_implicit_bias}
\min_{\W,\Hb}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\Delta_{y_i}\w_{y_i}-\Delta_c\w_c)^T\h_i \geq 1
\end{align}
\end{propo}

==> sections/implicit_bias.tex <==
\ct{@Ganesh: I moved the GD and logit regularization to Appendix, but feel free to reintroduce content in the main body as you see fit. Regarding logit regularization, where would this fit?}
\subsection{SVM solution is not a stationary direction of GD}

Let $\thetab := \vect(\W,\Hb) := [\w_1^T, \ldots, \w_k^T, \h_1^T, \ldots, \h_n^T]^T$ denote the vectorized representation of the embeddings and classifiers. Consider solving the unregularized  problem with gradient descent (GD) updates  $\thetab^{t+1} = \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)$, where $\Lc(\thetab^t):=\Lc(\W^t,\Hb^t)$ is the CE loss  in \eqref{eq:CE}. \cite{lyu2019gradient,ULPM} showed that the updates diverge in norm (i.e. $\|\thetab^t\|_2\rightarrow\infty$), but the normalized iterates $\thetab^t/\|\thetab^t\|_2$ converge to a  KKT point of \eqref{eq:SVM}. Since \eqref{eq:SVM} is nonconvex, it is unclear whether this point is a global optimum. Here, we use Theorem \ref{thm:global}  to show that a global minimizer $\hat\thetab$ of \eqref{eq:SVM} cannot be a converging direction of GD,  when classes are imbalanced. We start by formally defining the notion of a stationary direction below.

\begin{definition}[Stationary direction]
\label{defn:converging}
%We say a direction  $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction  of GD on $\Lc(\thetab)$ if and only if $\nicefrac{\nabla\Lc(\thetab)}{\|\nabla\Lc(\thetab)\|} = \nicefrac{-\thetab}{\|\thetab\|}$. 
We say $\thetab$ defines a stationary direction $\nbar{\thetab}=\nicefrac{\thetab}{\|\thetab\|}$
of GD on $\Lc(\thetab)$ if there exist constants $\kappa_1,\kappa_2>0$ such that $\nabla_\thetab\Lc(\kappa_1\thetab) = -\kappa_2\thetab$.
\end{definition}
%\gk{I think we have to refine the definition, or add assumptions- whether the relation should hold for all $\thetab$? What if for the same direction, some $\thetab$'s satisfy the condition while others do not?} \ct{Ok. Please  change and let's try to explain what's happening. Would something like the above work? I completed the proof and if I understand what you mean then it seems that the proof doesn't break.}
In words, a direction $\nicefrac{\thetab}{\|\thetab\|}$ is a stationary direction if the gradient descent update $\thetab^{+} = \thetab - \eta\nabla\Lc(\thetab)$ preserves this direction, i.e. $\nicefrac{\thetab^+}{\|\thetab^+\|_2}=\nicefrac{\thetab}{\|\thetab\|_2}$ , for any learning rate $\eta > 0$. 
\begin{definition}
	We say that $\nicefrac{\thetab}{\|\thetab\|}$ is a fixed direction under the GD update rule if and only if there exists an iteration $t$ such that $\frac{\thetab^{\tau}}{\|\thetab^{\tau}\|} = \frac{\thetab^{t}}{\|\thetab^{t}\|}, \quad\forall \quad\tau > t$.  \gk{tbd}
\end{definition}
\begin{lemma}
Suppose $\thetab$ is \emph{\underline{not}} a stationary direction of GD on $\Lc(\thetab)$. Then,
 	Under the GD update rule with finite learning rate $\eta >0$, $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is not a fixed direction 
	%\gk{to check if this term is good}
\end{lemma}
\begin{proof}
	Suppose $\thetab^t = \kappa\hat{\thetab}$ for some finite $\kappa >0$. Then, we show that $\thetab^{t+1}$, defined by an update of GD with a finite positive learning rate deviates from the direction $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$. Specifically, we will show that the projection of $\thetab^{t+1}$ onto the orthogonal complement of the subspace spanned by the vector $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ is non-zero. Let $\Pbf_{\hat{\thetab}}$ and $\Pbf_{\hat{\thetab}}^\perp$ be the matrices projecting a vector onto $\hat{\thetab}$ and the orthogonal complement of $\hat{\thetab}$, respectively. Then, from the GD update equation we have, 
	\begin{align*}
		\thetab^{t+1} &= \thetab^t - \eta\nabla_\thetab\Lc(\thetab^t)\\
		\implies \Pbf_{\hat{\thetab}}^\perp\thetab^{t+1} &= \Pbf_{\hat{\thetab}}^\perp\thetab^t + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\thetab^t)\right)\\
		&= \Pbf_{\hat{\thetab}}^\perp\kappa\hat{\thetab} + \eta \Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\kappa\hat{\thetab})\right)\\
		&= 0 + \frac{\eta\alpha_\kappa\kappa}{\alpha}\Pbf_{\hat{\thetab}}^\perp\left(-\nabla_\thetab\Lc(\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|\Pbf_{\hat{\thetab}}(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\right), \quad \text{where}\quad \beta = \frac{\eta\alpha_\kappa\kappa}{\alpha} > 0\\
		&= \beta^2\left(\|-\nabla_\thetab\Lc(\hat{\thetab})\|^2-\|(-\nabla_\thetab\Lc(\hat{\thetab}))\|^2\cos^2(\angle -\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)\\
		\implies \|\Pbf_{\hat{\thetab}}^\perp\thetab^{t+1}\|^2 &> 0, \quad \because \quad \angle \left(-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab}\right) \neq 0,\quad \text{from Proposition } \ref{propo:negative}.
	\end{align*}
\end{proof}
\gk{above, should we say explicitly that the angle is not 180 degrees either?}



With this definition, we now state the main result of this section. 



%\begin{assumption}\label{ass:align}
%\end{assumption}

\begin{propo}\label{propo:negative}
Assume imbalanced classes and $k>2$. Let $\hat\thetab=\vect(\What,\Hhat)$ be a global minimum of the non-convex SVM in \eqref{eq:SVM}. Then, $\nicefrac{\hat\thetab}{\|\hat\thetab\|}$ is \emph{not} a converging direction of GD on the CE loss.
\end{propo}
%\gk{I think we have to show this for all feasible scalar multiples of $\hat{\thetab}$? Related to how we define the convergence direction}

Proposition \ref{propo:negative} suggests that the KKT point to which GD converges to (in direction), is \emph{not} a global minimum of  \eqref{eq:SVM} when classes are imbalanced.
\footnote{Indeed, this statement can be formalized assuming that the GD path aligns with the gradients. While this statement is non-trivial, it has been proved (at least for $\eta\rightarrow0$) by \cite{} for binary data and we conjecture it to be true even for multiclass data (as already suggested by the results in \cite{}). 
 Specifically assume that $\lim_{t\rightarrow\infty}\inp{{\nbar{\thetab^t}}}{{-{\nbar{\nabla\Lc(\thetab^t)}}}}=1.$ If this is true, then Proposition \ref{propo:negative} and the gradient update rule yields  $\lim_{t\rightarrow\infty}\inp{\nbar{\thetab^t}}{\nicefrac{\hat\thetab}{\|\hat\thetab\|}}\neq1$. \ct{Check this!!!}% For the shake of contradiction assume this was not the case. Then, there exists $t_0$ such that for all $t\geq t_0$, $\|\nbar{\theta^t}-\nicefrac{\hat\thetab}{\|\hat\thetab\|}\|$
}. 
\ct{Also confirmed by our extended experiments in Figures ....} This is in stark to the balanced case, for which \cite{ULPM} showed that GD indeed converges to the global minimum of the non-convex SVM. Thus, \emph{even for a simple two-layer linear NN, it is in general \emph{not} true that GD converges to the global optimum of the corresponding max-margin optimization}. Specifically, while such a statement is always true for binary data as shown  by \cite{}, and for balanced multiclass data as shown by \cite{}, it fails for imbalanced multiclass data. 

\begin{remark} 
\ct{Check:}The proposition shows that the SVM solution is \emph{not} a converging direction of GD. From this, we can conclude that GD does not converge in that direction. On the other hand, note that showing a point $\thetab$ is a converging direction does \emph{not} imply that first-order methods necessariy converge in the direction of $\thetab$. This is because there might be a descending direction tangential to $\thetab$ (see for example \ref{unconstrained feature paper}).
\end{remark}



\paragraph{Proof.}
First, for arbitrary $\thetab$, denote the negative gradient of the CE loss as
	\begin{align}
		\g &:= -\nabla_\thetab\Lc(\thetab) = \sum_{i\in[n]}\sum_{c\neq y_i}\frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}\,\g_{i,c}\,,
	\end{align}
	where we denote the margins $s_{i,c} = (\w_{y_i}-\w_{c})^T\h_{i}$, and also, $\g_{i,c} = \nabla_\thetab s_{i,c}$. Specifically, using the shorthand $\alpha_{i,c} := \frac{e^{-s_{i,c}}}{1+\sum_{c'\neq y_i}e^{-s_{i,c'}}}$, we get $\g = \sum_{i\in[n]}\sum_{c\neq y_i}\alpha_{i,c}\g_{i,c}$. Here, note that $\g, \g_{i,c}, s_{i,c}$ are all functions of $\thetab$, but we suppress notation when clear from context.
	
Now, consider specific $\thetab = \kappa\hat{\thetab}$, where $\hat\thetab=\vect(\What,\Hhat)$, a global minimum of the non-convex SVM, and $\kappa >0$. From Theorem \ref{thm:global}\ref{thm:global_logits}, we know that $\hat\w_c^T\hat\h_i=\hat{z}_{ic}$ as defined in \eqref{eq:simplex}. Hence, the corresponding margins satisfy
\begin{align}
\forall i\in[n], c\neq y_i\,:\, s_{i,c}(\kappa\hat\thetab)=(\kappa\hat\w_{y_i}-\kappa\hat\w_{c})^T\kappa\hat\h_{i}=\kappa^2 \implies \alpha_{i,c}(\kappa\hat\thetab)=\alpha_\kappa>0,
\end{align}
Hence, $\g(\kappa\hat\thetab) = \alpha_\kappa\sum_{i\in[n]}\sum_{c\neq y_i}\g_{i,c}(\kappa\hat\thetab)$. In particular, evaluating $\g_{i,c}(\kappa\hat\thetab)=\nabla_\thetab s_{i,c}(\kappa\hat{\thetab})$ it follows that
\begin{subequations}\label{eq:grads_1}
	\begin{align}
\forall c \in [k]\,:\,~		-\nabla_{\w_{c}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\sum_{i: y_i=c}\hat\h_{i}-\sum_{i\in [n]}\hat\h_{i})\\
\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\kappa\hat\thetab) &= \alpha_\kappa\kappa(k\hat\w_{y_i}-\sum_{c\in[k]}\hat\w_{c}).
	\end{align}
\end{subequations}
We now compute the angle between $\thetab = \kappa\hat{\thetab}$ and $-\nabla_{{\thetab}}\Lc(\kappa\hat{\thetab})$.
%\noindent\textbf{Angle between parameter and gradient:}
It can be checked that the gradient at $\kappa\hat{\thetab}$ is related to the gradient at $\hat{\thetab}$ as follows:
\begin{align*}
	\forall c \in [K]\,:\,~	 \nabla_{\w_{c}}\Lc(\kappa\hat{\thetab}) &=  -\alpha_\kappa\kappa^2\left(Kn_c\hat{\h_c}-\sum_{c}n_{c'}\hat{\h_{c'}}\right) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\w_{c}}\Lc(\hat{\thetab})\\
	\forall i \in [n]\,:\,~	
	\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab}) &= \alpha_\kappa\kappa^2K\hat{\w_{y_i}} =\frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{\h_{i}}\Lc(\hat{\thetab})
\end{align*}	
where we used the following facts from Theorem \ref{thm:global} and $\alpha = \frac{\exp(-1)}{\left(1+(K-1)\exp(-1)\right)}$.
\begin{itemize}
	\item $\hat{\h}_{i} = \hat{\h}_{j}$ if $y_i = y_j$; denote $\hat{\h}_{i}$ by  $\hat{\h}_{c}$ when $y_i = c$
	\item $\sum_{c}\hat{\w}_c = 0$
\end{itemize}
Therefore, we get
$$\nabla_\thetab\Lc(\kappa\hat{\thetab}) = \frac{\alpha_\kappa\kappa^2}{\alpha}\nabla_{{\thetab}}\Lc(\hat{\thetab}),
$$
Now, computing the inner products,
\begin{align*}
	-\nabla_{\w_{c}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2\left((K-1)n_c\hat{\h}_c^T\hat{\w}_{c}-\sum_{c'\neq c}n_{c'}\hat{\h}_{c'}^T\hat{\w}_{c}\right)\\
	&= \alpha_\kappa\kappa^2\left[(K-1)n_c\frac{K-1}{K}+\frac{n-n_c}{K}\right]\\
	&= \frac{\alpha_\kappa\kappa^2}{K}\left[\left((K-1)^2-1\right)n_c+n\right]\\
	-\nabla_{\h_{i}}\Lc(\kappa\hat{\thetab})^T\kappa\hat{\w}_{c} &= \alpha_\kappa\kappa^2K\hat{\w}_{y_i}^T\h_{i}\\
	&= \alpha_\kappa\kappa^2(K-1)
\end{align*}
Combining in $\thetab$ notation, we have
\begin{align*}
	-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab} &= \alpha_\kappa\kappa^2\left[n(K-1)+n\frac{(K-1)^2-1}{K}+n\right]\\
	&= \frac{\alpha_\kappa\kappa^2n}{K}(2K^2-2K)\\
	&= 2\alpha_\kappa\kappa^2n(K-1)
\end{align*}
Thus, we get the following for the cosine of the angle between the parameter and negative gradient at $\kappa\hat{\thetab}$:
\begin{align*}
	\cos(\angle -\nabla_\thetab\Lc(\kappa\hat{\thetab}),\kappa\hat{\thetab}) &= \frac{-\nabla_\thetab\Lc(\kappa\hat{\thetab})^T\kappa\hat{\thetab}}{\|-\nabla_\thetab\Lc(\kappa\hat{\thetab})\|\kappa\hat{\thetab}\|}\\
	&= \frac{2\alpha_\kappa\kappa^2n(K-1)}{\frac{\alpha_\kappa\kappa^2}{\alpha}\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|}\\
	&= \frac{2n\alpha(K-1)}{\|-\nabla_\thetab\Lc(\hat{\thetab})\|\|\hat{\thetab}\|},
\end{align*}
which is independent of $\kappa$. This means that the angle between $\thetab$ and the negative gradient anywhere along the direction of $\hat{\thetab}$ remains a constant, irrespective of the magnitude of $\thetab$. Therefore, we can simplify the definition \ref{defn:converging} for $\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$ to be a stationary direction as there exists a $\gamma >0$ such that $\nabla\Lc(\hat{\thetab}) = -\gamma\hat{\thetab}$.
  


Next, suppose for the sake of contradiction that $\hat\thetab$ is a converging direction of GD. Following this (see Definition \ref{defn:converging}) and Equations \eqref{eq:grads_1}, there must exist $\kappa>0$ such that
\begin{subequations}\label{eq:grads_2}
	\begin{align}
\forall c \in [k]\,:\,~			-\nabla_{\w_{c}}\Lc(\hat\thetab) &= \alpha(k\sum_{i: y_i=c}\h_{i}-\sum_{i\in [N]}\h_{i}) = \gamma \w_{c} \label{eq:unreg_ce_grad_w_2}\\
	\forall i \in [n]\,:\,~		-\nabla_{\h_{i}}\Lc(\hat\thetab) &= \alpha(K\w_{y_i}-\sum_{c\in[k]}\w_{c}) = \gamma\h_{i}\label{eq:unreg_ce_grad_h_2}\,.
	\end{align}
\end{subequations}
Also, from Theorem \ref{thm:global}\ref{thm:global_W} and the fact that $\Zhat^T\ones_k =0$, we have that
$
\sum_{c\in[k]}\w_c=\What\ones_k = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\ones_k = 0 \footnote{In fact, this property can alternatively be deduces from \eqref{eq:unreg_ce_grad_w_2} by summing for all $c\in[k].$}.
$ Therefore, \eqref{eq:unreg_ce_grad_h_2} gives
	\begin{align}
	\forall i \in [n]\,:\,~	\alpha(k\hat\w_{y_i}) = \gamma\hat\h_{i}
		\implies   \hat\h_{i}=\gamma'\hat\w_{y_i}=\gamma'\What\y_i \nn,
	\end{align}
	for some constant $\gamma'>0$ and one-hot encoding vector $\y_i=\eb_{y_i}.$ 
	Therefore, letting $\Y=[\y_1,\ldots,\y_n]_{k\times n}$ be the one-hot label matrix, we conclude that 
\begin{align*}
	\Hhat^T\Hhat=\gamma'\Hhat^T\What\Y &\implies (\Zhat^T\Zhat)^{1/2}=\gamma'\Zhat^T\Y,
	\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\Y\Y^T\Zhat,
		\\
	&\implies \Zhat^T\Zhat=(\gamma')^2\Zhat^T\diag(n_1,n_2,\ldots,n_k)\Zhat,
	\\
	&\implies \Zhat^T\big(\Id_k - (\gamma')^2\diag(n_1,n_2,\ldots,n_k)\big)\Zhat=\zeromat_{n\times n},
	\\
	&\implies \Zhat^T\diag({1-(\gamma')^2{n_1}},{1-(\gamma')^2{n_2}},\ldots,{1-(\gamma')^2{n_k}})\Z=\zeromat_{n\times n},
\end{align*}
where, the first implication follows by Theorem \ref{thm:global}\ref{thm:global_logits} and \ref{thm:global_gram}. Denote for convenience $\delta_{c}=1-(\gamma')^2{n_c}, c\in[k]$ and $\Delta=\sum_{c\in[k]}\delta_c.$ Then, from the last line above, it must be that
\begin{align*}
	&\forall i\in[n]\,:\, \Big(1-\frac{1}{k}\Big)^2\delta_{y_i}^2+\frac{1}{k^2}\sum_{c\neq y_i}^k\delta_c^2 =0 \implies \big(k-1\big)^2\delta_{y_i}^2+(\Delta-\delta_{y_i}^2) = 0
	\\
		\implies &\forall c\in[k]\,:\, \big(k-1\big)^2\delta_{c}^2+(\Delta-\delta_{c}^2) = 0 		\implies k(k-2)\delta_{c}^2=-\Delta.
			\\
			\stackrel{k>2}{\implies} 
			&\forall c\in[k]\,:\,\delta_{c}^2=-\Delta \implies \delta_{1}=\delta_2=\ldots\delta_k \implies n_1=n_2=\ldots=n_k=n/k.
%		&\implies \forall i\in[n]\,:\, \big(k-1\big)^2(1-(\kappa')^2{n_{y_i}})=\sum_{c\neq y_i}^k (1-(\kappa')^2{n_c}) = k - (\kappa')^2(n-n_{y_i}) ,
%			\\
%		&\implies \forall i\in[n]\,:\,  (\kappa')^2\big((k-1)^2+1\big)n_{y_i} = (k-1)^2 - k +n
\end{align*}
But data were assumed imbalanced, so we arrived at a contradiction completing the proof. Note also that in the last line, we used the assumption $k>2$.

%We now note that, along the direction of the SVM solution $\hat{\thetab}$ it is sufficient to consider the following simplified definition of converging direction \ref{defn:converging}: We say $\hat{\thetab}$ defines a stationary direction $\nbar{\hat{\thetab}}=\nicefrac{\hat{\thetab}}{\|\hat{\thetab}\|}$
%of GD on $\Lc(\thetab)$ if and only if there exists a constant $\kappa_3>0$ such that $\nabla\Lc(\hat{\thetab}) = -\kappa_3\hat{\thetab}$, which is used in the proof of Proposition \ref{propo:negative}
%This is due to the fact that $\nabla_\thetab\Lc(\kappa_1\hat{\thetab}) = \nicefrac{\alpha'\kappa_1}{\alpha}\nabla_\thetab\Lc(\hat{\thetab})$, where $\alpha' = \frac{\exp(-\kappa_1^2)}{1+(K-1)\exp(-\kappa_1^2)}$ which is described in the discussion below. The observation further shows that the angle between $\kappa_1\hat{\thetab}$ and $-\nabla_{\thetab}\Lc(\kappa_1\hat\thetab)$ is independent of $\kappa_1$.

%\gk{Plots of angle as functions of R, K etc} 
\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm}
%		\caption{as a function of $R$}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[width=\linewidth]{Figures/angle_theta_mgrad_svm2}
%		\caption{Lorem ipsum}
	\end{subfigure}
	\caption{$\cos\left(\angle (-\nabla_\thetab\Lc(\hat{\thetab}),\hat{\thetab})\right)$ plotted against $R$ and $K$ respectively, with step imbalance on data. Note that the angle remains zero when $K=2$ or when $R=1$.}
\end{figure*}
%
%$$
%\forall c\in[k]\,,\, 1-(\kappa')^2{n_c} = 0 \implies n_1=n_2=\ldots=n_k.
%$$
%This contradicts our assumption that the dataset is imbalanced, completing the proof.


	%That is $\forall i\,:\, y_i=c$ the optimal feature $\hat\h_i$ aligns with the classifier $\hat\w_c$ of the corresponding class. 
	
	
%	Fix $i\in[n]$. Then from the display above and Theorem \ref{thm:global}\ref{thm:global_W},   
%	\begin{align}
%	\kappa'\hat\h_i = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}
%	Combining with Theorem \ref{thm:global}\ref{thm:global_Gram} (i.e. $\Hhat^T\Hhat=(\Zhat^T\Zhat)^{1/2}$), we conclude that
%	\begin{align}
%	\kappa'\Hhat^T\Hhat = \hat\w_{y_i} = \What\eb_{y_i} = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_{y_i}
%	\end{align}	
	
	
%	But again from Theorem \ref{thm:global}\ref{thm:global_W} 
%$\w_c=\What\eb_c = \Hhat(\Zhat^T\Zhat)^{-1/2}\Zhat^T\eb_c
%$

%	From \eqref{eq:h_opt} we have the relation between $\h_{i}^*$ and $\w_{y_i}^*$:
%	\begin{align*}
%		\hat\h_i = -\hat\W_{-y_i}\left(\Id+\ones\ones^T\right)\hat\lab_{y_i}.
%	\end{align*} 
%\gk{TBC}\ct{Need that $\w_{y_i}$ not aligned with $\h_i$.}



==> sections/intro.tex <==
%\ct{Change 'last-layer features' to 'embeddings'}
%\ct{Change 'universal' to 'invariant'}

%\subsection{Background, motivation and outlook.}
%\vspace{-0.2cm}
 {What are the unique structural properties of models learned by training deep neural networks to zero training error? Is there an \emph{implicit bias} towards solutions of certain geometry? How does this vary across training instances, architectures, and data? These questions are at the core of understanding the optimization landscape of deep-nets. Also, they are naturally informative about the role of models since different parameterizations might affect preferred geometries. Ultimately, such understanding makes progress towards explaining generalization of overparameterized models. %, as different global minima can have drastically different generalization properties. 

Recently, remarkable new progress in answering these questions has been made by \citet{NC}, who empirically discover and formalize the so-called \emph{Neural-collapse} (NC) phenomenon. NC describes  geometric properties of the learned embeddings (aka last-layer features) and of the classifier weights of deep-nets, trained with cross-entropy (CE) loss and \emph{balanced} data far into the zero training-error regime. The NC phenomenon produces a remarkably simple description of a particularly symmetric geometry: (i) The embeddings of each class collapse to their class mean (see \emph{\ref{NC}} property); and (ii) The class means align with the classifier weights and they form a simplex equiangular tight frame (see \emph{\ref{ETF}} property). Importantly, as noted by  \citet{NC}, this {simple} geometry appears to be ``cross-situational \emph{invariant}''
%\footnote{This ``universality" of NC properties across different instances of training, architectures and datasets is referred to as ``cross-situational invariant" structure in the original paper \cite{NC}. We adapt the term ``universal" structure here owing to its simplicity, otherwise the meaning is the same.} 
across different architectures and different \emph{balanced} datasets.
%\footnote{Albeit, the training speed at which the NC properties occur differs.}. 
%The second key feature is their simplicity translating to a remarkably symmetric geometry as follows: 
%% Specifically, they discovered empirically a set of three NC properties suggesting that, far into the interpolating regime, stochastic GD  converges to minimizers of the CE loss that are such that the learnt last-layer features and classifiers weights all collapse to a remarkably symmetric geometry as follows. 
%\textbf{(NC1)} The last-layer features converge  such that features within each class collapse to their mean vector. \textbf{(NC2)} Those different mean vectors  across classes are all of equal norm and maximally separated forming an Equiangular Tight Frame (ETF). \textbf{(NC3)} The classifier weights for each class align with their corresponding mean vectors; hence they also converge to the same ETF. %\cite{NC} experimentally confirmed these NC properties on balanced datasets, that is such that the number of training examples per class is equal. 
 %A notable feature of their discovery is that the phenomenon occurs consistently across different network architectures and different classification datasets; albeit the speed of convergence to the prescribed NC geometry differs.

In this paper, we study Neural collapse with {imbalanced} classes:
% that is when certain classes (minorities) have fewer training samples than others (majorities). Specifically, we ask: 
\emph{Is there a (ideally equally simple) description of the geometry that is invariant across \underline{class-imbalanced datasets}? 
%How do its specific characteristics change with the imbalance level?
}

\begin{figure}
	\begin{subfigure}{0.7\linewidth}
		\centering
		\includegraphics[scale=0.6]{figs/intro_seli4.pdf}
		\caption{\SELI~geometry;\\ $(10,\nicefrac{1}{2})$-STEP imbalance, $k=4$ classes}
		\label{fig:intro_SEL_seli}
	\end{subfigure}
\begin{subfigure}{0.24\linewidth}
	\centering
	\vspace{1cm}
\includegraphics[scale=0.52]{figs/etf_visual.pdf}
\captionsetup{width=0.9\linewidth}\caption{ETF~geometry;\\ $k=4$ balanced classes}
\label{fig:intro_SEL_etf}
\end{subfigure}
\caption{Visualization of the SELI and ETF geometries.}
\label{fig:intro_SEL}
\end{figure}



\vp
\noindent\textbf{Contributions.} We propose a new description capturing the geometric structure of learned-embeddings and classifier-weights on possibly \emph{class-imbalanced data}, which we call the \emph{Simplex-Encoded-Labels Interpolation}  \emph{\ref{SELI}} geometry. This new geometry is a generalization of the {ETF} geometry: It recovers the latter when data are balanced   {or when there are only two classes}, and also, unlike ETF, it remains invariant across different \emph{imbalance levels}. Importantly, it too, has a simple description: The matrix of learned logits interpolates a simplex-encoded label (SEL) matrix $\Zhat$, and, the individual  geometries of the embeddings and classifiers are determined by the SVD factors of this same \SEL~matrix. Because the particular arrangement of columns of the \SEL~matrix changes with the imbalance level, this also impacts the geometric arrangement of the embedding and classifier vectors.   {Overall, the norms and angles of these vectors admit simple closed-form expressions in terms of the imbalance characteristics and the number of classes.}
%See Ex.~ \ref{example:intro}

%\begin{example}\label{example:intro}
%For an illustration, 
We use an example to illustrate this. \Fig~\ref{fig:intro_SEL_seli} depicts the \SEL~matrix $\Zhat\in\R^{4\times 110}$ for a STEP-imbalanced $k=4$-class dataset with two majority classes of $50$ examples each, and, two minority classes of $5$ examples each. Each column of $\Zhat$ includes the $k$ learned logits for each one of the $110$ examples in the dataset. Each such column has exactly one entry equal to $1-1/k=0.75$ and  three entries equal to $-1/k=-0.25$. The corresponding geometry of the embeddings and classifiers, shown in the 3D plot, is found by an SVD of $\Zhat$: the left eigenvectors determine the classifiers and the right ones the embeddings. Note that $\Zhat$ is rank 3, hence the geometry is  3D. Since embeddings collapse to their class means (see \emph{\ref{NC}} property), we only show the four {\color{blue}class-mean embeddings} and the corresponding four {\color{red}classifiers}. Two of each correspond to majorities (``$\bullet$'' marker) and two to minorities (``$+$'' marker).   {The radii of the two concentric spheres are equal to the norms of the minority classifiers (red sphere) and of the minority embeddings (blue sphere), respectively. Note that the norms of minorities and majorities are different, and so are the angles. Moreover, the classifiers are \emph{not} aligned with the embeddings. Overall, the geometry  is different compared to the ETF geometry seen in the balanced case, which is shown in Fig. \ref{fig:intro_SEL_etf}.}   {What remains invariant across class-imbalances is that the logits (i.e. inner products between classifiers and embeddings) only take values either $1-1/k$  or  $-1/k$, so that the logit matrix is equal to the \SEL~matrix. Equivalently, the learned model interpolates the simplex-encoding of the labels.}
%However, note that all the margins with respect to any class equal $(1-1/k)-(-1/k)=1;$ thus, they are all the same.}
% Also, norms and in-between angles are different for minorities and majorities. 
%\end{example}

Below we explain the conception of this geometry and our contributions in  detail. The initial major challenge was: \emph{Assuming a class-imbalance-invariant geometry exists, how to find  it?} %Specifically, we focus and analyze the UFM trained with CE loss and imbalances.

%  adapt the ansatz from the literarature \cite{} that the UFM predicts the correct geometry. Yet, the geometry of solutions to the UFM has not been yet characterized when data are imbalanced. Neither has it been studied wether it correctly predicts the geometry of solutions to training deep nets. 
%
%
%To gain more insights on the NC phenomenon a series of subsequent works introduced and analytically studied a simplified two-layer proxy model \cite{mixon2020neural}, called the Unconstrained Feature Model (UFM) \footnote{\ct{Talk about different names to this}}. Here, the first and second layers of the UFM correspond each to the last-layer features and the classifier weights of the neural net. These works have shown that when data are balanced, then the solution found by GD on the UFM is fully consistent with and offers a potential theoretical explanation of the NC properties. We note that despite its simple formulation, empirical risk minimization on the UFM involves minimizing a non-convex objective. Thus, characterizing the properties of solutions found by GD on this non-convex landscape is a priori a challenging task.

%\noindent$\bullet$~
To answer this question, we adopted the \emph{Unconstrained Feature Model (UFM}) previously introduced in the literature as a  two-layer proxy model to theoretically justify neural collapse \cite{mixon2020neural,fang2021exploring,zhu2021geometric}. Motivated by deep-learning practice and by studies on implicit bias of gradient descent (GD) for unregularized CE minimization, we analyze the geometry of solutions to an unconstrained-features Support Vector Machines (UF-SVM) problem. We prove, for STEP-imbalanced data, any solution of the UF-SVM follows the SELI geometry. Thus, the learned end-to-end model always interpolates a simplex labels encoding. We show that \emph{\ref{ETF}}$\implies$\emph{\ref{SELI}}. However, \emph{\ref{SELI}}$\not\implies$\emph{\ref{ETF}} unless classes are balanced or there is just two of them ($k=2$). %For balanced data, we show that the SELI geometry recovers the ETF geometry. \ct{We quantify properties of the SELI geometry for imbalanced data}

%\noindent$\bullet$~
Next, we analyze training of the UFM with ridge-regularized CE. Unlike previous studies, we find in the presence of imbalances that regularization matters as it changes the geometry of solutions. In fact, we show that there is \emph{no} finite regularization that leads to the  SELI geometry. However, we also show that as regularization vanishes, the solutions do interpolate the \SEL~matrix (after appropriate normalization.) Finally, 
%converge (in direction) to the SELI geometry.  
%$\noindent$\bullet$~
we show that the SELI geometry differs from the minority-collapse phenomenon \cite{fang2021exploring}, since the latter does not correspond to solutions with zero training error. In fact, we show for minority collapse that: (i)  It does \emph{not} occur for small finite regularization   {and finite imbalance ratio, and (ii) It occurs asymptotically for vanishing regularization, but only asymptotically as the imbalance ratio grows.}   %(See Fig.~\ref{fig:UFM_nuc_norm_lambda_margin} and SM due to space constraints.)



%\noindent$\bullet$~
We numerically test convergence to the proposed SELI geometry in both synthetic and real class-imbalanced datasets. For different imbalance levels, the learned geometries approach the SELI geometry significantly faster compared to the ETF geometry. See \Fig~\ref{fig:intro_CIFAR}.
However, we also observe that convergence \emph{worsens} with increasing level of imbalance. A plausible theoretical justification is that as we show regularization plays critical role under imbalances. We also consistently get better convergence rate for the classifiers. We believe our observations strongly motivate further investigations regarding potential frailties of ``asymptotic'' implicit bias characterizations and how these might vary in multiclass and possibly imbalanced settings. 

\input{sections/IntroFigure}



\vp
\noindent\textbf{Why imbalanced?}~~Investigating structural geometric properties under data imbalances is important for the following reasons. First, data-imbalances appear in various learning tasks more often than not. Thus, it is relevant understanding what deep neural networks learn in these settings. Second, the previously discovered, perfectly symmetric, ETF geometry only holds when the data distribution is  itself symmetric. This naturally raises a question, which we answer here: when this data symmetry breaks, is it still possible to characterize potentially non-symmetric geometries? We argue this result is nontrivial, particularly so because the new geometry is richer than the ETF as it is parameterized by not only the number of classes, but also by the imbalance ratio and the fraction of minorities. Third, while previous work has shown the simplified unconstrained-features model is powerful to predict the exact geometry when classes are balanced, it is not a priori known whether the model is also able to predict the corresponding geometry when classes are imbalanced. Our paper shows this to be the case and also uncovers several unique features when data are imbalanced (e.g., it shows that the UFM solution depends on the regularization parameter.) Finally, it is known that data imbalances affect generalization since vanilla training with cross-entropy loss results in poor generalization for minority classes. We envision that understanding how the properties of the learnt geometries vary for minorities versus majorities could help create links between structural results and generalization towards explaining the effectiveness of existing or inspiring new techniques for mitigating imbalances.

\input{sections/IntroTable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\paragraph{Contributions.} Perhaps  the most remarkable ingenuity behind the experimental demonstration of NC by Papyan et al., is the conception of a simple formula for the underlying geometry of the class embeddings and classifier weights. For balanced data, this geometry is fully described in terms of an ETF \cite{NC}. This is confirmed experimentally by measuring the cosine similarity between the Gram matrices of the classifiers/features and the ETF Gram matrix, and showing that it approaches one with increasing number of SGD iteration (see for example Figure \ref{fig:}\ct{ADD Figure!}). On the contrary, for imbalanced data, NC2 and NC3 do not hold: neither the classifier weights, nor the features, form an ETF. This can be confirmed experimentally by showing that the same cosine similarity distance to ETF does \emph{not} converge to one; see Figure \ref{fig:} \ct{ADD Figure!}. Moreover, as seen in Figure \ref{fig:} \ct{ADD Figure!} the distance to ETF appears to change with the level of imbalance. So, how to find a formula characterizing the geometry with imbalaned data (assuming that such a universal geometry characterization exists)? To do this, we adapt the ansatz from the literarature \cite{} that the UFM predicts the correct geometry. Yet, the geometry of solutions to the UFM has not been yet characterized when data are imbalanced. Neither has it been studied wether it correctly predicts the geometry of solutions to training deep nets. 
%
%
%Our contributions can be outlined as follows.
%
%\textbf{Benign-{non}convexity of UFM remains true under imbalances.} Recall that the UFM is a non-convex optimization. However, previous work by Zhu et al., Ji et al.,... \cite{zhu2021geometric,ULPM} has shown that the non-convexity is benign in that all stationary points are either strict saddles (hence, can be avoided by most first-order methods), or, they are global optima. Moreover, these global optima are characterized by solving a convex relaxation corresponding to nuclear-norm regularized CE minimization. 
%
%We formulate the \emph{\ref{SELI}} property and prove that it characterizes the UF-SVM solution for both balanced and imbalanced data. Specifically, we show that \emph{\ref{SELI}}$\equiv$\emph{\ref{ETF}} for balanced data, but \emph{\ref{SELI}}$\neq$\emph{\ref{ETF}} under imbalances. 


		% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ %


%Another very closely related line of research is quickly emerging around the so-called Neural Collapse (NC) phenomenon discovered by \cite{NC}.  Specifically, \cite{NC} discovered empirically a set of NC properties suggesting that in the terminal phase of deep-learning training with CE loss and no explicit regularization, the last-layer features and classifiers weights, all collapse to a very specific and symmetric geometry. Namely, the features learnt by the deepnet at the last layer converge to a geometry such that features within each class collapse to their mean vector and the different mean vectors  across  classes are of equal norm and maximally separated. Also, the classifier weights for each class align with the corresponding mean vector. Since the appearance of \cite{NC}, there have been several works that confirm the findings of \cite{} and also attempt to theoretically justify based on a so-called unconstrained feature model. Most of these works focus on balanced datasets. Instead, we undertake an investigation of NC with imbalances, which leads to the following findings.


%\section{Introduction}

%Understanding the optimization landscape of deep neural networks has been a major focus of the research community over the past few years. Driven by current deep-learning practice, it has been of particular interest identifying the types of models that are learnt when training architectures with a number of parameters that far exceeds the size of the training set and without explicit regularization. 

%
%
%When training deep nets with a number of parameters that far exceeds the size of the training set and without explicit regularization, first-order optimizers, such as (stochastic) gradient descent (GD), usually have no trouble in finding---one of the many---global minimizers of the emprical risk. Instead, the challenging question is: \emph{What are the unique properties of the specific minimizer preferred by the optimizer? That is, is there an \emph{implicit bias} of towards certain types of minimizers?} This question is at the core of understanding non-convex optimization in overparameterized settings. Also, it is naturally informative about the role of the model architecture since different parameterizations might lead to different preferred solutions. Ultimately, it is conceivable that understanding the geometry of preferred solutions is also related to generalization, as different global minima can have drastically different generalization properties. 


%\gk{Introduction to training overparameterized models, phenomemon of neural collapse, intro to imbalance}
%Overparameterized learning models have a large number of parameters that are learned from a relatively fewer number of training examples. Many modern machine learning architectures belong in this category of models. In the training of overparameterized neural networks for supervised learning, specifically, classification using gradient based algorithms on popular loss functions like the cross-entropy (CE) loss, the phenomenon of neural collapse has been observed. Neural collapse has been used to refer to the emergence of a certain degeneracy and symmetry in the learned features and classifier weights. In many recent studies, analytical explanations for neural collapse are shown with various models. In this work, we study the neural collapse properties when the training dataset has label-imbalance, i.e., the training data has an unequal number of examples belonging to different classes.
%
%Label-imbalance is frequently encountered in practice. A major aspect of studying the problem of label-imbalance is to design algorithms that have equitable test performance despite the disparity in the training examples. A study of neural collapse under label-imbalance could shed light on the dynamics of optimizing a model with a certain loss function and thus help design better algorithms.

%\section{Neural Collapse Properties}

==> sections/logit_regularization.tex <==
%\subsection{Logit Regularization}
\ct{@Ganesh: Please write this in notation consistent with what we have above.}
Consider the following regularization to the CE loss:
\begin{align}
	\Lc_\text{LogReg}(\W,\Hb) = \sum_{i\in[N]} \log\Big(1+\sum_{c\neq y_i}e^{-(\w_{y_i}-\w_c)^T\h_i}\Big) + \frac{\lambda}{2}\|\W^T\Hb\|_F^2.\label{eq:LogRegCE_ncvx}
\end{align}
In the above problem, the regularization is on the logit-matrix $\Z=\W^T\Hb$. We show in the proposition below that with such ``logit-regularization", for any positive strength of the regularizer, the optimal solution yields a global scaling of the SEL matrix $\Zhat$ as its logit-matrix. This further means that all the margins are equal. This is in contrast with the optimal solution of the ridge-regularized ERM with finite regularizer strength, wherein the optimal solution is different in direction from the SEL matrix.
\begin{propo}
	The logit-regularized CE loss can be lower bounded as below:
	\begin{align*}
		\Lc_\text{LogReg}(\W,\Hb) \geq \alpha(\rho^*),
	\end{align*}
	where $\alpha(\rho) = \log\Big(1+(K-1)\exp\Big(-\rho\sqrt{\frac{K}{N(K-1)}}\Big)\Big)+\frac{\lambda}{2}\rho^2$, $\rho^*$ is the solution to the following equation:
	\begin{align*}
		\rho &= \frac{\beta}{\lambda}\frac{(K-1)\exp(-\beta\rho)}{1+(K-1)\exp(-\beta\rho)}, \quad \text{where}\quad \beta = \sqrt{\frac{K}{N(K-1)}}
	\end{align*}
	The minimum margin $q_{min}$ is upper bounded as 
	$$
	q_{min} \leq {\beta\rho^*}
	$$
	The bounds are achieved by a $(\W,\Hb)$ if and only if the following conditions are satisfied, with $\Z = \W^T\Hb$:
	\begin{enumerate}
		\item $\|\z_i\| = \|\z_j\|, \quad \forall i,j \in [N]$
		\item $z_{i,l} = z_{i,k}, \quad \forall l,k \neq y_i $
		\item $\z_i = -\delta \ab, \quad \text{for some}\quad \delta > 0 \quad \text{where}\quad \mathbf{a} = [1\quad 1\quad ... (1-K)\quad ... 1]$
		\item $\|\Z\|_F = \rho^*$ 
	\end{enumerate}

	
\end{propo}

\begin{proof}
	Consider the following convex problem:
	\begin{align}
		\Lc_\text{LogReg}(\Z) &= \sum_{i\in[N]} \log\Big(1+\sum_{c\neq y_i}e^{-(Z_{y_i,i}-Z_{c,i})}\Big) + \frac{\lambda}{2}\|\Z\|_F^2,\label{eq:LogRegCE_cvx}\\
		&= \Lc_\text{CE}(\Z) + \frac{\lambda}{2}\|\Z\|_F^2 \nonumber
	\end{align}
	
	We can lower bound the contribution of each example to the loss in \eqref{eq:LogRegCE_cvx} as below:
	\begin{align*}
		\Lc_\text{CE}(\z, y) &= \log\Big(1+\sum_{c\neq y}\exp(z_c-z_y)\Big)\\
		&\geq \log\Big(1+(K-1)\exp\Big(\sum_{c\neq y}\frac{z_c-z_y}{K-1}\Big)\Big)\\
		&= \log\Big(1+(K-1)\exp\Big(\frac{\sum_{c}z_c-Kz_y}{K-1}\Big)\Big)\\
		&\geq \log\Big(1+(K-1)\exp\Big(-\frac{\|\mathbf{a}\|\|\z\|}{K-1}\Big)\Big), \quad \text{where}\quad \mathbf{a} = [1\quad 1\quad ... (1-K)\quad ... 1]\\
		&= \log\Big(1+(K-1)\exp\Big(-\sqrt{\frac{K}{K-1}}\|\z\|\Big)\Big),
	\end{align*}
	
	Now, using the above in the overall logit-regularized CE loss, we have that
	\begin{align}
		\Lc_\text{LogRegCE}(\Z) &\geq \log\Big(1+(K-1)\exp\Big(-\rho\sqrt{\frac{K}{N(K-1)}}\Big)\Big)+\frac{\lambda}{2}\rho^2 := \alpha(\rho), \rho := \|\Z\|_F > 0 \label{eq:logreg_cvx_lb_rho}
	\end{align}
	
	Eqn \eqref{eq:logreg_cvx_lb_rho} gives a lower bound on the logit-regularized loss, as a function of $\|\Z\|_F$, for any logit-matrix $\|\Z\|$. Further, minimizing $\alpha(\rho)$ over $\rho > 0$, we get $\alpha(\rho^*)$ as an absolute lower bound on $\Lc_\text{LogRegCE}(\Z)$, where $\rho^*$ is the solution of the following equation \gk{ToDo: investigate the nature of this function, whether it has a unique solution, how to find analytically etc}
	\begin{align}
		\rho = \frac{\beta}{\lambda}\frac{(K-1)\exp(-\beta\rho)}{1+(K-1)\exp(-\beta\rho)}, \quad \text{where}\quad \beta = \sqrt{\frac{K}{N(K-1)}}
	\end{align}
	Therefore, for any $(\W,\Hb)$, we have the following lower bound on $\Lc_\text{LogRegCE}(\W,\Hb)$
	\begin{align}
		\Lc_\text{LogRegCE}(\W,\Hb) &\geq \alpha(\rho^*)\label{eq:logreg_ncvx_lb}
	\end{align}
	\subsubsection*{Conditions for equality of \eqref{eq:logreg_ncvx_lb}}
	For any $(\W,\Hb)$, let $\Z = \W^T\Hb$. The lower bound $\eqref{eq:logreg_ncvx_lb}$ is achieved with equality if \gk{check whether if and only if} the following conditions hold:
	\begin{enumerate}
		\item $\|\z_i\| = \|\z_j\|, \quad \forall i,j \in [N]$
		\item $z_{i,l} = z_{i,k}, \quad \forall l,k \neq y_i $
		\item $\z_i = -\delta \ab, \quad \text{for some}\quad \delta > 0$ 
	\end{enumerate}
	The SVM solution, normalized so as to have $\|\W^T\Hb\|_F=\rho^*$ satisfies the above conditions for equality, therefore is a global minimum of $\Lc_\text{LogRegCE}(\W,\Hb)$. %\gk{Can we show this analytically?}
	
\end{proof}

\subsection{Effect of Logit Regularization}

==> sections/outlook.tex <==
%\vspace{-0.25cm}
We propose \emph{\ref{SELI}} as the class-imbalance-invariant geometry of classifiers and embeddings learnt by overparameterized models when trained beyond zero training error. We arrive at it after showing that the UF-SVM global minimizers follow this geometry. Subsequently, we conjecture that: (C1) GD on the UFM leads to solutions approaching the SELI geometry asymptotically in the number of epochs; (C2) training of deep-nets beyond zero training error learns models that approach the SELI geometry. 

Statement (C1) is a conjecture and does not follow from Theorem~\ref{thm:SVM}. This is because GD is only known to converge to KKT points of the non-convex UF-SVM \cite{lyu2019gradient,ULPM}, which are not necessarily global minima.  Thus, while Proposition~\ref{propo:reg_path} combined with the benign landscape of the corresponding ridge-regularized minimization, as well as, our experiments suggest its validity, the conjecture remains to be further investigated.\footnote{Relying on \citep{ji2020directional}, \citet{vardi2021margin} showed gradient flow  finds global minimizers in deep linear nets. However, these only apply to binary classification. We show that interesting behaviors might occur (e.g. in the role of regularization and geometry) when $k>2$ and $R>1$ calling  further studies.} We also note that convergence rates appear slower with increasing imbalance levels; a feature which is interesting to study further. 

Regarding conjecture (C2), we deem our experiments encouraging: the classifiers' and embeddings' geometries get closer to the SELI geometry as neural-network training progresses. Specifically, the Gram matrices $\G_\W$ and $\G_\Hb$ of the classifiers and embeddings, respectively, align increasingly better with their SELI counterparts $\Vb\Lambdab\Vb^T$ and $\Ub\Lambdab\Ub^T$; see \Fig~\ref{fig:intro_CIFAR}. Also, \Fig~\ref{fig:norm_ratio_exp_W} shows that Lemma \ref{lem:norms} is able to make predictions regarding the norms of majorities versus minorities. We note that, similar to the UFM experiments, convergence appears slower for larger imbalance ratios. Also, we observe better convergence for classifiers compared to embeddings {and for norm predictions compared to angle predictions}. Overall, we hope our results motivate further experimental investigations, especially since data imbalances appear frequently across applications. 
 %\new{In our experiments, we use optimization-parameter choices (e.g. learning rate, weight-decay, momentum) that are consistent with previous works in the literature.} 

 Beyond that, we believe that further similar studies on identifying geometric structures of learned embeddings and classifiers could offer new perspectives on generalization. Our results could pave that way since they uncover different geometries (aka SELI for different $R$ values), each leading to different generalization (worse for increasing $R$ \cite{byrd2019effect}). %On one hand, CE on balanced data leads to ETF geometry, and, is known to generalize well. On the other hand, CE on imbalanced data changes the geometry, and, is known to achieve poor generalization  in terms of (say) balanced error \cite{byrd2019effect}. since having access to different geometries  each leading to different generalization might help uncovering connections between train geometries and generalization. 
 Relatedly, we envision that further such studies lead to algorithmic contributions in  imbalanced deep-learning as they can facilitate studying the implicit-bias effect of CE adjustments and post-hoc techniques tailored to imbalanced data \cite{TengyuMa,Menon,CDT,KimKim,kang2020decoupling,kini2021label,li2021autobalance}.

%
%\ct{
%Future work:
%\begin{itemize}
%\item general imbalance (beyond step)
%\item other losses, e.g. square loss?
%\end{itemize}
%}

%\paragraph{Rethinking implicit bias: Imbalance trouble}  \ct{needs rewriting}A series of works that examine the implicit bias of gradient descent (and of its variants, such as stochastic GD, gradient flow, etc.) yield characterizations of the preferred minimizer that roughly take the following format: the model weights found by GD converge to a KKT point of an optimization program that minimizes a certain norm of the weights subject to an interpolation constraint. In the simplest and cleanest setting of a linear model trained with either square-loss or cross-entropy, the resulting optimization is convex and minimizes the $\ell_2$ norm of the weights subject to either an interpolation constraint or a linear separability constraint \cite{}. For example, GD on cross-entropy loss in a linear setting converges (in direction) to the max-margin classifier \cite{}. We note that in general nonlinear settings, the norm that is minimized can depend on the model architecture \cite{}. Perhaps more importantly, beyond the linear setting, the resulting optimization program is non-convex. This naturally raises the question of whether the KKT point preferred by GD is a global minimizer. Our first finding shows that the answer is in general negative even in the simplest setting beyond the standard linear model, that of a 2-layer linear network:
% 
%\begin{finding}
%Consider training of a 2-layer linear network with gradient flow (GF) on cross-entropy (CE) loss without explicit regularization. There exists multiclass imbalanced dataset such that the global minimizer of the (non-convex) max-margin optimization is \emph{not} a convergence direction of GF.
%\end{finding}
%\begin{figure}[ht!]
%	\centering
%	\includegraphics[width=\linewidth]{Figures/G_errors_CE}
%\end{figure}
%\ct{@Ganesh: One plot -two curves. One for balanced. one for imbalanced. distance to G cvx (which corresponds to global optimum) over epochs. In the LPM model.}


%We believe these questions are important since data imbalances appear more frequently, than not, across applications \cite{}. Beyond that, answering these questions might offer a new perspective in better understanding potential connections of NC to generalization. On the one hand, CE entropy on balanced data leads to the symmetric geometry characterized by NC1--3, and also, it is known to achieve good generalization. On the other hand, as we will see, the presence of imbalances drastically changes the geometry, and also, it is known to achieve poor generalization, measured in terms of (say) balanced error \cite{}. Having access to different geometries that each leads to different generalization levels might shed light in understand wether a connection between NC and generalization can be formalized. Relatedly, we envision that our study leads to algorithmic contributions in imbalanced learning with overparameterized models as it can be used to study changes to NC geometry when training with losses other than CE that are tailored to imbalanced data.

==> sections/proof_of_global_opt.tex <==
\paragraph{Proof.} Let $ \mathrm{p}_* = \|\Hhat\|_F^2+\|\What\|_F^2$ denote the optimal cost of the non-convex SVM in \eqref{eq:svm_original}. First, we constraint the feasible set over $\Hb$ in \eqref{eq:svm_original} to the following compact set:
\begin{align}\label{eq:artificial_H}
\Hc := \left\{\Hb\in\R^{d\times n}\,:\, \exists \{\w_c\}_{c\in[k]} \text{ s.t. } (\w_{y_i}-\w_c)^T{\h_i} \geq 1, \quad \|\Hb\|_F^2\leq C \right\},
\end{align}
with $C>\mathrm{p}_*$ being a large constant whose exact value will be determined later in the proof. This additional constraint, does \emph{not} change the optimal set of \eqref{eq:svm_original}. 
To see this note that any minimizer $\Hhat$ of \eqref{eq:svm_original} is feasible (hence $\exists \{\w_c\}_{c\in[k]} \text{ s.t. } (\w_{y_i}-\w_c)^T{\hat{\h}_i} \geq 1$), and, also satisfies $\|\Hhat\|_F^2\leq \|\Hhat\|_F^2+\|\What\|_F^2=\mathrm{p}_*<C.$


Next, consider the optimization over $\W$ for fixed $\Hb\in\Hc$:
\begin{align}\label{eq:W_primal}
\mathrm{p}_*^{\Hb} := \min_{\W} \frac{1}{2}\|\W\|_2^2\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1,~i\in[n], c\neq y_i.
\end{align}
The dual of this takes the following standard form:
\begin{align}\label{W_dual}
\mathrm{d}_*^{\Hb} := \max_{\la_{ic}\geq 0, i\in[n], c\neq y_i}~~\sum_{i\in[n]}\Big(\sum_{c\neq y_i}\la_{ic}\Big)-\frac{1}{2}\sum_{c\in[k]}\Big\|\sum_{i: y_i=c}\Big(\sum_{ c\neq y_i}\la_{ic}\Big) \h_i - \sum_{i: y_i\neq c}\la_{ic}\h_i\Big\|_2^2.
\end{align}
Instead of this standard form, it is convenient to work with an alternative representation that makes the dual objective separable. To arrive to this, define dual variables $\beta_{ic}, i\in[n], c\in[k]$ such that
\begin{align}
\beta_{ic}=\begin{cases}
\sum_{c'\neq y_i}\la_{ic'}, &y_i=c,
\\-\la_{ic},&y_i\neq c.
\end{cases}
\end{align}
Specifically, for $c\in[k]$, set $\betab^{(c)}=[\betab_{1c},\ldots,\betab_{nc}]^t\in\R^{n}$. Also, let $\zhat^{(c)}=[\hat{x}_{1c},\ldots,\hat{z}_{nc}]^t\in\R^{n}, c\in[k]$ denote the rows of the matrix $\Zhat$. 
Then, it can be checked that the dual problem can be equivalently written as follows:
\begin{align}
\mathrm{d}_*^{\Hb} := &\max_{\beta_{ic}, i\in[n], c\in[k]}~~\sum_{c\in[k]}\big(\betab^{(c)}\big)^T\zhat^{(c)}-\frac{1}{2}\|\Hb\betab^{(c)}\|_2^2 \nn\\
&\text{subject to}~~~ \beta_{iy_i} = -\sum_{c\neq y_i}
\beta_{ic}, \qquad \betab^{(c)}\odot\zhat^{(c)}\geq 0 \label{eq:W_dual2}
\end{align}
Now, note that the optimization in \eqref{eq:W_primal} is clearly convex and trivially satisfies Slater's conditions (feasibility is ensured since $\Hb\in\Hc$). Hence, strong duality holds. In particular, $\mathrm{p}_*^{\Hb}=\mathrm{d}_*^{\Hb}$ and also 
\begin{align}\label{eq:strong_duality}
\forall c\in[k]\,:\,~~ \w_c^* = \sum_{i:y_i=c}\Big(\sum_{c'\neq y_i}\la^*_{ic}\Big)\h_i - \sum_{i:y_i\neq c}\la^*_{ic}\h_i  = \sum_{i\in[b]}\beta_{ic}\h_i = \Hb (\betab^{(c)})^* \implies \W^*=\Hb\Bb^*,
\end{align}
where $\W^*$ is the minimizer in \eqref{eq:W_primal} and $\Bb^*:=[(\betab^{(1)})^*,\ldots,(\betab^{(k)})^*]\in\R^{n\times k}$ is a dual optimal in \eqref{eq:W_dual2}.

With these, we now return to the joint optimization over both $\W$ and $\Hb$ in \eqref{eq:svm_original}, which we repeat here for convenience
\begin{align}
\mathrm{p}_* = \min_{\Hb\in\Hc,\W}~\frac{1}{2}\|\W\|^2+ \frac{1}{2}\|\Hb\|^2
\quad\quad\text{sub. to}\quad (\w_{y_i}-\w_c)^T\h_i \geq 1,~i\in[n], c\neq y_i.
\end{align}
%Note that there is no loss of generality in constraining the optimization over $\Hb$ to the set 
Using the duality above and denoting for convenience
$$
\Bc:=\big\{ \Bb = [\beta_{ic}]_{i\in[n],c\in[k]}\,:\, \beta_{iy_i} = -\sum_{c\neq y_i}
\beta_{ic}, \quad \beta_{ic}\hat{z}_{ic}\geq 0 \big\} = \big\{ \Bb \in\R^{n\times k}:\, \Bb\ones_{k}=0,  \quad \Bb\odot\Zhat \geq 0 \big\},
$$
and 
\begin{align}\label{eq:S}
\Sc:=\big\{ \Bb\in\R^{n\times k}\,: \Id_n\succeq \Bb\Bb^T\big\} = \big\{ \Bb\in\R^{n\times k}\,: \|\Bb\|_2\leq 1\big\},
\end{align}
the original optimization is equivalent to:
\begin{align}
\mathrm{p}_*  &= \min_{\Hb\in\Hc}~\max_{\Bb\in\Bc}~~ \tr(\Zhat\Bb) + \frac{1}{2} \tr\Big(\Hb^T\Hb\big(\Id_{n}-\Bb\Bb^T\big)\Big)\nn\\
&=\min_{\Hb\in\Hc}~\max_{\Bb\in\Bc\cap\Sc}~ \tr(\Zhat\Bb) + \frac{1}{2} \tr\Big(\Hb^T\Hb\big(\Id_{n}-\Bb\Bb^T\big)\Big)\label{eq:sion}\\
&=\max_{\Bb\in\Bc\cap\Sc}~\min_{\Hb\in\Hc}~ \tr(\Zhat\Bb) + \frac{1}{2} \tr\Big(\Hb^T\Hb\big(\Id_{n}-\Bb\Bb^T\big)\Big)\nn\\
%&=\max_{\Bb\in\Bc\cap\Sc}~\min_{\G_H\in\left\{\G=\Hb^T\Hb \,:\, \Hb\in\Hc\right\}}~ \tr(\Zhat\Bb) + \frac{1}{2} \tr\Big(\G_H\big(\Id_{n}-\Bb\Bb^T\big)\Big)\nn\\
&=\max_{\Bb\in\Bc\cap\Sc}~ \tr(\Zhat\Bb).\label{eq:dual}
\end{align}
In the second line above, we used the fact that for $\Bb\not\in\Sc$, $\min_{\Hh}\tr(\Hb^T\Hb \big(\Id_{n}-\Bb\Bb^T\big) )\succeq 0$ . In the third line, we used Sion's min-max theorem to change the order of min and max after noting that (i) the objective in \eqref{eq:sion} is convex in $\Hb$ and concave in $\Bb$; (ii) the two constraint sets $\Hc$ and $\Bc\cap\Sc$ are convex; (iii) the constraint set $\Hc$ is compact. To find \eqref{eq:dual}, we used again that $\Hb^T\Hb\succeq 0$ and $\tr(\M_1\M_2)\geq 0$ for $\M_1\succeq0,\M_2\succeq 0$.

To continue consider the following relaxation of the minimization in \eqref{eq:dual}:
\begin{align}
\mathrm{q}_* = \max_{\Bb\in\Sc}~ \tr(\Zhat\Bb).
\end{align}
Recalling the definition of the set $\Sc$ in \eqref{eq:S} it follows immediately that $\mathrm{q}_*=\|\Zhat\|_*$ with minimizer $\widetilde\Bb=(\Zhat^T\Zhat)^{-1/2}\Zhat^T$. We now show that 
\begin{align}\label{eq:feasibility}
\widetilde\Bb=(\Zhat^T\Zhat)^{-1/2}\Zhat^T\in\Bc.
\end{align}
Indeed, note that $\widetilde\Bb\ones_k=(\Zhat^T\Zhat)^{-1/2}\Zhat^T\ones_k=0$. Also, it holds that $\widetilde\Bb\odot \Zhat^T = ((\Zhat^T\Zhat)^{-1/2}\Zhat^T)\odot \Zhat^T\geq 0 $ \ct{Why?}

Thus, $\widetilde\Bb$ is feasible in \eqref{eq:dual}, which gives that it is also a minimizer therein and also $\mathrm{p}_*=\mathrm{q}_*=\|\Zhat\|_*.$

%\implies \forall i\in[n]\,:\,\sum_{c\in[k]}\beta_{ic}=0.$

%The optimization above is convex and Slater's conditions are satisfied (e.g. $\Bb=0$ is strictly feasible). Thus, strong duality holds and the following KKT conditions are necessary and sufficient for optimality


==> sections/results.tex <==
\subsection{Theory}
\begin{enumerate}
	\item Whether balanced or imbalanced, the global minimizers of the ridge-regularized non-convex ERM are also global minimizers of nuclear-norm-regularized convex ERM.
	\item For balanced data, with any strength of ridge regularization, a normalized global minimum of the non-convex problem is equivalent to the two layer SVM solution. The normalized logit matrix is equal to $\Zhat$
	\item For imbalanced data, the global solution of ridge-regularized non-convex ERM is sensitive to the regularization strength
	\item For imbalanced data, there does not exist a finite regularization strength, such that the 2-layer SVM solution satisfies the first-order optimality conditions: \ref{propo:negative}
	\item With ridge regularization, the optimization landscape of the non-convex ERM is benign, irrespective of imbalance. Specifically, any critical point of the non-convex ERM is either a global minimum or has a negative curvature. What is the tightest sufficient condition?
	\item Irrespective of the imbalance, the ridge regularized ERM, as $\lambda\rightarrow 0$, has a logit matrix converging to $\Zhat$. In numerical experiments on UFM, this is not always apparent, but needs appropriate learning rate scheduling. With imbalance, this is even more difficult.
	\item Characterization of global solution of 2-layer SVM with imbalance. Solution satisfies NC1, while having different NC2/3 properties. We compute the angles between classifiers, feature means, and calculate the logit matrix. The logit matrix is a scaling of $\Zhat$: \ref{thm:global}
	\item Logit regularized non-convex ERM yields $\Zhat$ as the global solution for any $\lambda_\text{LogReg}$. 
	\item Ridge regularized non-convex ERM corresponds to nuclear-norm regularized convex ERM with corresponding $\lambda$, whose global minimum varies with $\lambda$. Logit regularized non-convex ERM corresponds to ridge-regularized convex ERM with corresponding $\lambda_\text{LogReg}$, whose normalized solution is $\Zhat$ for any $\lambda_\text{LogReg} > 0$.
	\item Relationship with minority collapse: 
	\item 
\end{enumerate}
\subsection{Empirical: UFM}
\begin{enumerate}
	\item Under separation constraints, $\arg\min_{\Z} \|Z\|_* = \arg\min_{\Z} \|Z\|_F$
\end{enumerate}
\subsection{Empirical: DeepNets}
\begin{enumerate}
	\item NC1 holds, NC2/3 hold with different characterization, sensitive to ridge regularization strength
	\item With finite ridge regularization, under SGD, angles and logits converge close to the UFM solution
	 
\end{enumerate}



\paragraph{Implicit bias.} A series of works that examine the implicit bias of gradient descent (and of its variants, such as stochastic GD, gradient flow, etc.) yield characterizations of the preferred minimizer that roughly take the following format: the model weights found by GD converge to a KKT point of an optimization program that minimizes a certain norm of the weights subject to an interpolation constraint. In the simplest and cleanest setting of a linear model trained with either square-loss or cross-entropy, the resulting optimization is convex and minimizes the $\ell_2$ norm of the weights subject to either an interpolation constraint or a linear separability constraint \cite{}. For example, GD on cross-entropy loss in a linear setting converges (in direction) to the max-margin classifier \cite{}. We note that in general nonlinear settings, the norm that is minimized can depend on the model architecture \cite{}. Perhaps more importantly, beyond the linear setting, the resulting optimization program is non-convex. This naturally raises the question of whether the KKT point preferred by GD is a global minimizer. Our first finding shows that the answer is in general negative even in the simplest setting beyond the standard linear model, that of a 2-layer linear network:
 
\begin{finding}
Consider training of a 2-layer linear network with gradient flow (GF) on cross-entropy (CE) loss without explicit regularization. There exists multiclass imbalanced dataset such that the global minimizer of the (non-convex) max-margin optimization is \emph{not} a convergence direction of GF.
\end{finding}
\begin{figure}[ht!]
	\centering
	\includegraphics[width=\linewidth]{Figures/G_errors_CE}
\end{figure}
\ct{@Ganesh: One plot -two curves. One for balanced. one for imbalanced. distance to G cvx (which corresponds to global optimum) over epochs. In the LPM model.}

\paragraph{Neural collapse.} Another very closely related line of research is quickly emerging around the so-called Neural Collapse (NC) phenomenon discovered by \cite{NC}.  Specifically, \cite{NC} discovered empirically a set of NC properties suggesting that in the terminal phase of deep-learning training with CE loss and no explicit regularization, the last-layer features and classifiers weights, all collapse to a very specific and symmetric geometry. Namely, the features learnt by the deepnet at the last layer converge to a geometry such that features within each class collapse to their mean vector and the different mean vectors  across  classes are of equal norm and maximally separated. Also, the classifier weights for each class align with the corresponding mean vector. Since the appearance of \cite{NC}, there have been several works that confirm the findings of \cite{} and also attempt to theoretically justify based on a so-called unconstrained feature model. Most of these works focus on balanced datasets. Instead, we undertake an investigation of NC with imbalances, which leads to the following findings.

\begin{finding} When training imbalanced datasets:
\begin{enumerate}
 \item the classifier weights do \emph{not} align with the learnt feature means of the corresponding class \ct{@Vala: This is for vala plot cosine (again balanced vs unbalanced). IMPORTANT: same number of overall data.}
 \begin{figure}[ht!]
 	\centering
 	\begin{subfigure}[b]{\linewidth}
 		\centering
 		\includegraphics[width=\textwidth]{Figures/NC3_Fail_plot}
 		\includegraphics[width=\textwidth]{Figures/NC3_Fail_plot_10Class}
 		\caption{$\frac{1}{k} \Sigma_{c = 0}^K || \frac{W_c}{||W_c||} - \frac{\dot{M}_c}{||\dot{M}_c||} ||$}
 	\end{subfigure}%
 	
 	\begin{subfigure}[b]{\linewidth}
 		\centering
 		\includegraphics[width=\textwidth]{Figures/NC3_Cos_Fail_plot}
 		\includegraphics[width=\textwidth]{Figures/NC3_Cos_Fail_plot_10Class}
 		\caption{$ \frac{1}{k} \Sigma_{c = 0}^K  \frac{W_c \cdot \dot{M}_c}{||W_c|| \cdot ||\dot{M}_c||} $}
 	\end{subfigure}%
 	\caption{Classifiers do not converge to train class mean: 
 	\newline
 	(fig a) To compare the geometry of the classifiers and class-means we measure the per class normalized classifier elements to their respective class-mean counterparts by comparing the norms. The figure indicates that the convergence does not happen in the case of imbalance. (See section ? for more information).  
 	\newline
 	(fig b) To compare the geometry of the classifiers and class-mean we measure the cosine angle between the weight and mean vectors on a per class basis. The cosine values are then averaged across the classes and reported above. For the balanced case, the cosine almost goes to 1 indicating convergence. However the vectors divergence with higher imbalance ratios.  (See section ? for more information).   }
 \end{figure}

 \item weights of different classes are not of equal norm. Specifically, minority classes get smaller  norms. Same for class means(?) 
\begin{figure}[ht]
	\centering
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/W_Norm_Ratios_Fail}
		\includegraphics[width=\textwidth]{Figures/W_Norm_Ratios_Fail_10Class}
		\caption{Classifier Norm Ratio = $\overline{|| W_{maj} ||} \; / \; \overline{|| W_{min} ||}$}
	\end{subfigure}%
	
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/M_Norm_Ratios_Fail}
		\includegraphics[width=\textwidth]{Figures/W_Norm_Ratios_Fail_10Class}
		\caption{Class-Mean Norm Ratio = $\overline{|| M_{maj} ||} \; / \; \overline{|| M_{min} ||}$}
	\end{subfigure}%

	\caption{Majority vs minority norms are not equal: Comparison between the norm of classifiers for majority and minority classes indicates that for imablanced data, the ratio of the norms does not converge to 1. In the case of classifiers, the majority classes tend to have larger classifier norms when compared to their minority counterparts (fig a). In contrast, for the case of class means (fig b), the minority classes tend have larger norms compared to the majority classes. Results are averaged across 3 iterations of full training with different sets of 4 classes taken from CIFAR10 and MNIST respectively (See section ? for more information). }
\end{figure}
 \end{enumerate}
 Moreover, unlike the case of balanced data, the geometry found by gradient descent is different from the optimal one under the unconstrained feature model. 
\end{finding}

Does the LPM model predict the deep net behavior? 



\begin{finding}
Margins are not same. But they become same with logit regularization. 
\begin{figure}[ht]
	\centering
	\begin{subfigure}[b]{\linewidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Min_Margin_Stdev_Conv}
		\caption{Margin Convergence = $\text{stdev}_{c\in[k]} ( \min_{c'\neq c \in [0,K]} [(\w_{c} - \w_{c})^T \mub_c ])/\text{Avg}_{c\in[k]} ( \min_{c'\neq c \in [0,K]} [(\w_{c} - \w_{c})^T \mub_c ])$}
		
		\includegraphics[width=\textwidth]{Figures/Min_Margin_Stdev_Conv_10Class}
		\caption{Margin Convergence = $\text{stdev}_{c\in[k]} ( \min_{c'\neq c \in [0,K]} [(\w_{c} - \w_{c})^T \mub_c ])/\text{Avg}_{c\in[k]} ( \min_{c'\neq c \in [0,K]} [(\w_{c} - \w_{c})^T \mub_c ])$}
		
	\end{subfigure}%

	\caption{Min-Margin divergence with imbalance: The standard deviation between min-margins appear to suggest a general convergence of the margins. However this convergence is less prominent in the case of step imbalance (See section ? for more information).   }
\end{figure}
\end{finding}


 \ct{Old comments: 
 \textbf{How the size of training set affects NC}Is NC purely an optimization phenomenon? How does the size of the training set affect convergence? \textbf{Weight decay} Convergence is faster with small, but non-zero, weight decay; \textbf{Compare $\G_\W$ and $\G_\Hb$:} Show that with CE, $\G_\W$ is "worse" compared to $\G_\Hb.$ Can we see this from. \textbf{Majority vs minority norms of features/weights} 
 }

